Mining Temporal Evolution of Knowledge Graph and Genealogical Features for Literature-based Discovery Prediction

Literature-based knowledge discovery process identifies the important but implicit relations among information embedded in published literature. Existing techniques from Information Retrieval and Natural Language Processing attempt to identify the hidden or unpublished connections between information concepts within published literature, however, these techniques undermine the concept of predicting the future and emerging relations among scientific knowledge components encapsulated within the literature. Keyword Co-occurrence Network (KCN), built upon author selected keywords (i.e., knowledge entities), is considered as a knowledge graph that focuses both on these knowledge components and knowledge structure of a scientific domain by examining the relationships between knowledge entities. Using data from two multidisciplinary research domains other than the medical domain, capitalizing on bibliometrics, the dynamicity of temporal KCNs, and a Long Short Term Memory recurrent neural network, this study proposed a framework to successfully predict the future literature-based discoveries - the emerging connections among knowledge units. Framing the problem as a dynamic supervised link prediction task, the proposed framework integrates some novel node and edge-level features. Temporal importance of keywords computed from both bipartite and unipartite networks, communities of keywords, built upon genealogical relations, and relative importance of temporal citation counts used in the feature construction process. Both node and edge-level features were input into an LSTM network to forecast the feature values for positive and negatively labeled non-connected keyword pairs and classify them accurately. High classification performance rates suggest that these features are supportive both in predicting the emerging connections between scientific knowledge units and emerging trend analysis.

==> Other_pages/background.tex <==
\section{Background}
\setlabel{Background}{subsec:bckgnd}
\subsection {Knowledge Evolution and Dynamic KCN}
\setlabel{Keyword co-occurrence network}{subsec:kcn}
Currently, scientific knowledge creation is  dynamic and interdisciplinary in nature where different avenues of research converge and new connections emerge among disjoint and existing areas of science ~\cite{pan2012evolution}.
This knowledge is generally an incremental process except few revolutionary and fundamental changes.
The development and evolution of science and technology create new knowledge from the previously accumulated and ubiquitous information ~\cite{lee2009approach}.
New hypotheses are being postulated by encompassing existing scientific concepts from multiple domains.
Agusti Canals ~\cite{canals2005knowledge} pointed out that the diffusion of scientific knowledge can be mapped into a network structure where knowledge propagates via interactions among networked agents.  
A knowledge graph (network) is a specific kind of knowledge representation technique that uses a semantic network structure where vertices are keywords  links represent their causal relationships ~\cite{popping2003knowledge}
Statistically significant and non-trivial co-occurrence patterns of keywords not only represent their semantic affinity ~\cite{montemurro2013keywords} and relatedness ~\cite{schulz2014semantic} but also their causal relationships ~\cite{mcnorgan2007feature}.
Therefore, using the extracted, cleaned, and processed keywords, as described above, dynamic Keyword Co-occurrence Networks (KCNs) were constructed for each year in 2008-2015.
% As mentioned earlier in section \ref{sec:data_acquisition}, we omitted the year 2007 as a training year.
KCN is defined as an undirected network $G(V, E)$ where nodes $V$ is the set of author selected keywords and $E$ is the set of edges where each edge represents the co-appearance of two keywords in the same article. 
Multiple such co-appearances define the edge weights which is ignored in this study.
% The number of connections or frequency of co-occurrences between two nodes is the corresponding edge weight. 
Dynamic KCNs are the temporal networks $G_t = (v_t, e_t)$ for time period $t = 1,2,...,T$ where 
$v_t$ is the set of nodes or keywords and 
$e_t$ is the set of edges connecting the set of keywords $v_t \in V$ at time $t$. 
These edges at time $t$ can be new or recurring. 
Table \ref{table:node-edge state} provides statistics of the number of nodes (keywords) and edges (co-occurrences) per year in both datasets.
% Given a time series of KCN, we formulate a supervised link prediction problem in dynamic networks to predict the co-occurrences of author selected keywords in future articles. 

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=.95\textwidth]{{framework}.png}
%     \caption{Dynamic link prediction framework to predict future co-appearances of author-selected keywords, extracted from the scientific literature, to support literature based knowledge discovery}
%     %\caption*{A note}
%     \label{fig:framework}
% \end{figure}

\ignore{
\begin{table}[!h]
\centering
\begin{threeparttable}
\caption{Node and edge statistics of co-word networks for the two datasets}
\label{table:node-edge state}
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}}lrrrrrr}
\toprule
Dataset name & Year	& $E_T$ &  $E_{T+1}$ & $V_T$	& Positively-labeled edges & Negative-labeled Edges 		\\
\midrule
\multirow{8}{*}{$G_{s}$} & 2008 &  773 & & 459 & \multirow{7}{*}{1441}&\multirow{7}{*}{590195}		\\
		    & 2009	&  620		&  		  & 191		&				    & 			\\
		    & 2010	&  674		&  		  & 133		&				    & 			\\
		    & 2011	&  799		&  		  & 95		&				    & 			\\
		    & 2012	&  808		&  		  & 79		&				    & 			\\
		    & 2013	&  977		&  		  & 90		&				    & 			\\
		    & 2014	&  826		&  		  & 46		&				    & 			\\\cmidrule{2-7}
		    & 2015	&  		 	&  5142	  & 1093		&				    & 			\\
\midrule

\multirow{8}{*}{$G_{o}$}& 2008	&  10285 &  & 2357& \multirow{7}{*}{14203}&\multirow{7}{*}{8033692}	\\
			& 2009	&  8894 	&  		  & 531		& 					&				\\
			& 2010	&  9210 	&  	      & 276		&				    & 			\\
			& 2011	&  9970 	& 	      & 120		&				    & 			\\
			& 2012	&  556	 	&  		  & 61		&				    & 			\\
			& 2013	&  530	 	&  		  & 28		&				    & 			\\
			& 2014	&  13892 	&  		  & 652		&				    & 			\\\cmidrule{2-7}
			& 2015	&  		 	&  21610  & 4025	&				    & 			\\
\bottomrule
\end{tabular*}
\begin{tablenotes}
\item $E_T$ represents the set of edges in the training phase (2008-2014) and $E_{T+1}$ represents edges in the test phase (2015). $E_T$ is the set of all nodes (Keywords) common between training and test years. Positively labeled edges are those non-connected keyword-pairs from training phase appeared in the test phase whereas negatively labeled edges are all other keyword-pairs non-existent in both training and test phase.
\end{tablenotes}
\end{threeparttable}
\end{table}
}
In Table \ref{table:gr_ke}, we present the basic statistics of the evolutionary patterns observed in dynamic KCN for both $G_o$ and $G_s$. 
The dynamicity of keyword co-occurrences denotes that new research topics, hypotheses or directions emerge over time through co-appearances of existing keywords.
% Needless to mention here that the author selected keywords which are voluntarily hand-picked by the scholars of the scientific articles denote these topics.
% These emergence can justify the existing relations between keywords strengthening the exercised hypotheses, spawn new avenues of research directions, or engender new postulations. 
Three different scenarios can be observed in dynamic KCN: 

\begin{table}[!h]
\centering
\begin{threeparttable}
\caption{Evolutionary statistics of nodes (author selected keywords) and edges (co-occurrences in the same article) for two datasets in this study. $V_t$ = keywords in year $t$, $V_{n}$ = new keywords each year, $V_{o}$ = old keywords from the previous year(s), $E$ = edges, $E_{o \leftrightarrow o}$ = recurring edges between $v\in V_{o}$, $E{}'_{o\leftrightarrow o}$ = new edges between  $v\in V_{o}$, $E_{n \leftrightarrow o}$ = edges between $v\in V_{o}$ and $v\in V_{n}$, $E_{n \leftrightarrow n}$ = edges between $v\in V_{n}$. The term `old' in a particular year denotes the set of keywords appeared in previous year(s)}
\label{table:gr_ke}
\begin{tabular*}{\textwidth}{l@{\extracolsep{\fill}}rrrrrrrrr}
\toprule
{} &  year &    $V_t$ &   $V_{n}$ &   $V_{o}$ &     $E$ &  $E_{o \leftrightarrow o}$ &   $E{}'_{o\leftrightarrow o}$ & $E_{n \leftrightarrow o}$ & $E_{n \leftrightarrow n}$ \\
\midrule
$G_{s}$   &  2007 &   857 &  857 &     0 &  1486 &      0 &      0 &     0 &  1486 \\
     &  2008 &   968 &  572 &   396 &  1690 &    144 &    530 &   777 &   239 \\
     &  2009 &   978 &  438 &   540 &  1587 &    202 &    609 &   636 &   140 \\
     &  2010 &  1000 &  332 &   668 &  1648 &    264 &    800 &   483 &   101 \\
     &  2011 &  1172 &  345 &   827 &  2264 &    387 &   1166 &   599 &   112 \\
     &  2012 &  1240 &  279 &   961 &  2399 &    271 &   1524 &   531 &    73 \\
     &  2013 &  1328 &  272 &  1056 &  2715 &    424 &   1692 &   539 &    60 \\
     &  2014 &  1367 &  291 &  1076 &  2728 &    500 &   1605 &   502 &   121 \\
     &  2015 &  1262 &  157 &  1105 &  2347 &    512 &   1530 &   235 &    70 \\
\midrule
$G_{o}$  &  2007 &  3207 &  3207 &     0 &  15725 &      0 &      0 &     0 &  15725 \\
    &  2008 &  3515 &  1217 &  2298 &  16826 &   3167 &   8995 &  4336 &    328 \\
    &  2009 &  4206 &  1709 &  2497 &  21122 &   4515 &   9091 &  6695 &    821 \\
    &  2010 &  4696 &  1152 &  3544 &  24093 &   6578 &  13154 &  4094 &    267 \\
    &  2011 &  5059 &   658 &  4401 &  29261 &   6514 &  19962 &  2698 &     87 \\
    &  2012 &  5426 &   364 &  5062 &  32663 &   9944 &  20900 &  1744 &     75 \\
    &  2013 &  5418 &    77 &  5341 &  32076 &  11702 &  19987 &   382 &      5 \\
    &  2014 &  4283 &   738 &  3545 &  22410 &   6522 &  12386 &  3251 &    251 \\
    &  2015 &  4466 &   367 &  4099 &  23606 &   8043 &  13860 &  1548 &    155 \\
\bottomrule
\end{tabular*}
\begin{tablenotes}
\item 
\end{tablenotes}
\end{threeparttable}
\end{table}

As observable in Table  \ref{table:gr_ke}, firstly, new edges emerge each year when new keywords co-appear in articles.
Secondly, new keywords form edge with old (existing) keywords (appeared in previous years).
Finally, edges are formed in a year between two old keywords from the previous year(s), where these old keywords appeared in different articles but not co-appeared in the same article.
The term `old' in any particular year $t$ denotes the set of keywords appeared in year(s) prior to $t$. \eg, in $G_{s}$ for the year 2010, the number of $V_{o}$ is $668$ which denotes that out of $V_t=1000$ keywords in 2010, $668$ keywords appeared within 2007-2009. 
% Emergence of new keywords each year do not always necessarily represent the discovery of new scientific concept(s). 
It is observable from the table that the number of new keywords normally decreases.
When a new hypothesis gains considerable attentions in the subsequent years, the related keywords become significant.
This fact prompts expansion of these keywords' degree through new or recurring relations. 
Besides, new relations between old keywords $E_{o \leftrightarrow o}$ were found to be dominating which is the generic trend in inter-disciplinary research. 
Further, the growth of edges in  $E{}'_{o\leftrightarrow o}$ implies that most new hypotheses emerge across existing keywords, topics, and/or concepts. 
Conversely, sporadic nature of new hypothesis generation across new keywords can be observed through the decreasing number of edges in $E_{n\leftrightarrow n}$.
Delayed consumption of new concepts by the scientific communities can be attributed as a cause. 
In case of $E_{n\leftrightarrow o}$, we observed that a lot of edges are formed with the most central keywords within the research domain which is true for knowledge network evolution (preferential attachment). 

% \section{Background}
% \setlabel{Background}{subsec:bckgnd}
\subsection {Knowledge Evolution and Dynamic KCN}
\setlabel{Keyword co-occurrence network}{subsec:kcn}
Currently, scientific knowledge creation is  dynamic and interdisciplinary in nature where different avenues of research converge and new connections emerge among disjoint and existing areas of science ~\cite{pan2012evolution}.
This knowledge is generally an incremental process except few revolutionary and fundamental changes.
The development and evolution of science and technology create new knowledge from the previously accumulated and ubiquitous information ~\cite{lee2009approach}.
New hypotheses are being postulated by encompassing existing scientific concepts from multiple domains.
Agusti Canals ~\cite{canals2005knowledge} pointed out that the diffusion of scientific knowledge can be mapped into a network structure where knowledge propagates via interactions among networked agents.  
A knowledge graph (network) is a specific kind of knowledge representation technique that uses a semantic network structure where vertices are keywords  links represent their causal relationships ~\cite{popping2003knowledge}
Statistically significant and non-trivial co-occurrence patterns of keywords not only represent their semantic affinity ~\cite{montemurro2013keywords} and relatedness ~\cite{schulz2014semantic} but also their causal relationships ~\cite{mcnorgan2007feature}.
Therefore, using the extracted, cleaned, and processed keywords, as described above, dynamic Keyword Co-occurrence Networks (KCNs) were constructed for each year in 2008-2015.
% As mentioned earlier in section \ref{sec:data_acquisition}, we omitted the year 2007 as a training year.
KCN is defined as an undirected network $G(V, E)$ where nodes $V$ is the set of author selected keywords and $E$ is the set of edges where each edge represents the co-appearance of two keywords in the same article. 
Multiple such co-appearances define the edge weights which is ignored in this study.
% The number of connections or frequency of co-occurrences between two nodes is the corresponding edge weight. 
Dynamic KCNs are the temporal networks $G_t = (v_t, e_t)$ for time period $t = 1,2,...,T$ where 
$v_t$ is the set of nodes or keywords and 
$e_t$ is the set of edges connecting the set of keywords $v_t \in V$ at time $t$. 
These edges at time $t$ can be new or recurring. 
Table \ref{table:node-edge state} provides statistics of the number of nodes (keywords) and edges (co-occurrences) per year in both datasets.
Given a time series of KCN, we formulate a supervised link prediction problem in dynamic networks to predict the co-occurrences of author selected keywords in future articles. 

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=.95\textwidth]{{framework}.png}
%     \caption{Dynamic link prediction framework to predict future co-appearances of author-selected keywords, extracted from the scientific literature, to support literature based knowledge discovery}
%     %\caption*{A note}
%     \label{fig:framework}
% \end{figure}

\ignore{
\begin{table}[!h]
\centering
\begin{threeparttable}
\caption{Node and edge statistics of co-word networks for the two datasets}
\label{table:node-edge state}
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}}lrrrrrr}
\toprule
Dataset name & Year	& $E_T$ &  $E_{T+1}$ & $V_T$	& Positively-labeled edges & Negative-labeled Edges 		\\
\midrule
\multirow{8}{*}{$G_{s}$} & 2008 &  773 & & 459 & \multirow{7}{*}{1441}&\multirow{7}{*}{590195}		\\
		    & 2009	&  620		&  		  & 191		&				    & 			\\
		    & 2010	&  674		&  		  & 133		&				    & 			\\
		    & 2011	&  799		&  		  & 95		&				    & 			\\
		    & 2012	&  808		&  		  & 79		&				    & 			\\
		    & 2013	&  977		&  		  & 90		&				    & 			\\
		    & 2014	&  826		&  		  & 46		&				    & 			\\\cmidrule{2-7}
		    & 2015	&  		 	&  5142	  & 1093		&				    & 			\\
\midrule

\multirow{8}{*}{$G_{o}$}& 2008	&  10285 &  & 2357& \multirow{7}{*}{14203}&\multirow{7}{*}{8033692}	\\
			& 2009	&  8894 	&  		  & 531		& 					&				\\
			& 2010	&  9210 	&  	      & 276		&				    & 			\\
			& 2011	&  9970 	& 	      & 120		&				    & 			\\
			& 2012	&  556	 	&  		  & 61		&				    & 			\\
			& 2013	&  530	 	&  		  & 28		&				    & 			\\
			& 2014	&  13892 	&  		  & 652		&				    & 			\\\cmidrule{2-7}
			& 2015	&  		 	&  21610  & 4025	&				    & 			\\
\bottomrule
\end{tabular*}
\begin{tablenotes}
\item $E_T$ represents the set of edges in the training phase (2008-2014) and $E_{T+1}$ represents edges in the test phase (2015). $E_T$ is the set of all nodes (Keywords) common between training and test years. Positively labeled edges are those non-connected keyword-pairs from training phase appeared in the test phase whereas negatively labeled edges are all other keyword-pairs non-existent in both training and test phase.
\end{tablenotes}
\end{threeparttable}
\end{table}
}
In Table \ref{table:gr_ke}, we present the basic statistics of the evolutionary patterns observed in dynamic KCN for both $G_o$ and $G_s$. 
The dynamicity of keyword co-occurrences denotes that new research topics, hypotheses or directions emerge over time through co-appearances of existing keywords.
% Needless to mention here that the author selected keywords which are voluntarily hand-picked by the scholars of the scientific articles denote these topics.
% These emergence can justify the existing relations between keywords strengthening the exercised hypotheses, spawn new avenues of research directions, or engender new postulations. 
Three different scenarios can be observed in dynamic KCN: 

\begin{table}[!h]
\centering
\begin{threeparttable}
\caption{Evolutionary statistics of nodes (author selected keywords) and edges (co-occurrences in the same article) for two datasets in this study. $V_t$ = keywords in year $t$, $V_{n}$ = new keywords each year, $V_{o}$ = old keywords from the previous year(s), $E$ = edges, $E_{o \leftrightarrow o}$ = recurring edges between $v\in V_{o}$, $E{}'_{o\leftrightarrow o}$ = new edges between  $v\in V_{o}$, $E_{n \leftrightarrow o}$ = edges between $v\in V_{o}$ and $v\in V_{n}$, $E_{n \leftrightarrow n}$ = edges between $v\in V_{n}$. The term `old' in a particular year denotes the set of keywords appeared in previous year(s)}
\label{table:gr_ke}
\begin{tabular*}{\textwidth}{l@{\extracolsep{\fill}}rrrrrrrrr}
\toprule
{} &  year &    $V_t$ &   $V_{n}$ &   $V_{o}$ &     $E$ &  $E_{o \leftrightarrow o}$ &   $E{}'_{o\leftrightarrow o}$ & $E_{n \leftrightarrow o}$ & $E_{n \leftrightarrow n}$ \\
\midrule
$G_{s}$   &  2007 &   857 &  857 &     0 &  1486 &      0 &      0 &     0 &  1486 \\
     &  2008 &   968 &  572 &   396 &  1690 &    144 &    530 &   777 &   239 \\
     &  2009 &   978 &  438 &   540 &  1587 &    202 &    609 &   636 &   140 \\
     &  2010 &  1000 &  332 &   668 &  1648 &    264 &    800 &   483 &   101 \\
     &  2011 &  1172 &  345 &   827 &  2264 &    387 &   1166 &   599 &   112 \\
     &  2012 &  1240 &  279 &   961 &  2399 &    271 &   1524 &   531 &    73 \\
     &  2013 &  1328 &  272 &  1056 &  2715 &    424 &   1692 &   539 &    60 \\
     &  2014 &  1367 &  291 &  1076 &  2728 &    500 &   1605 &   502 &   121 \\
     &  2015 &  1262 &  157 &  1105 &  2347 &    512 &   1530 &   235 &    70 \\
\midrule
$G_{o}$  &  2007 &  3207 &  3207 &     0 &  15725 &      0 &      0 &     0 &  15725 \\
    &  2008 &  3515 &  1217 &  2298 &  16826 &   3167 &   8995 &  4336 &    328 \\
    &  2009 &  4206 &  1709 &  2497 &  21122 &   4515 &   9091 &  6695 &    821 \\
    &  2010 &  4696 &  1152 &  3544 &  24093 &   6578 &  13154 &  4094 &    267 \\
    &  2011 &  5059 &   658 &  4401 &  29261 &   6514 &  19962 &  2698 &     87 \\
    &  2012 &  5426 &   364 &  5062 &  32663 &   9944 &  20900 &  1744 &     75 \\
    &  2013 &  5418 &    77 &  5341 &  32076 &  11702 &  19987 &   382 &      5 \\
    &  2014 &  4283 &   738 &  3545 &  22410 &   6522 &  12386 &  3251 &    251 \\
    &  2015 &  4466 &   367 &  4099 &  23606 &   8043 &  13860 &  1548 &    155 \\
\bottomrule
\end{tabular*}
\begin{tablenotes}
\item 
\end{tablenotes}
\end{threeparttable}
\end{table}

As observable in Table  \ref{table:gr_ke}, firstly, new edges emerge each year when new keywords co-appear in articles.
Secondly, new keywords form edge with old (existing) keywords (appeared in previous years).
Finally, edges are formed in a year between two old keywords from the previous year(s), where these old keywords appeared in different articles but not co-appeared in the same article.
The term `old' in any particular year $t$ denotes the set of keywords appeared in year(s) prior to $t$. \eg, in $G_{s}$ for the year 2010, the number of $V_{o}$ is $668$ which denotes that out of $V_t=1000$ keywords in 2010, $668$ keywords appeared within 2007-2009. 
% Emergence of new keywords each year do not always necessarily represent the discovery of new scientific concept(s). 
It is observable from the table that the number of new keywords normally decreases.
When a new hypothesis gains considerable attentions in the subsequent years, the related keywords become significant.
This fact prompts expansion of these keywords' degree through new or recurring relations. 
Besides, new relations between old keywords $E_{o \leftrightarrow o}$ were found to be dominating which is the generic trend in inter-disciplinary research. 
Further, the growth of edges in  $E{}'_{o\leftrightarrow o}$ implies that most new hypotheses emerge across existing keywords, topics, and/or concepts. 
Conversely, sporadic nature of new hypothesis generation across new keywords can be observed through the decreasing number of edges in $E_{n\leftrightarrow n}$.
Delayed consumption of new concepts by the scientific communities can be attributed as a cause. 
In case of $E_{n\leftrightarrow o}$, we observed that a lot of edges are formed with the most central keywords within the research domain which is true for knowledge network evolution (preferential attachment). 

\subsection {Preferential Attachment and Recursive Centrality}
\setlabel{Recursive centrality}{sec:rec_centrality}
The generation of author selected keywords is governed by the inherent rules of scholarly communication which is also known as preferential attachment ~\cite{zhao2018ranking}.
In citation-based scholarly communication, few articles within a research area will draw most attention and subsequently acquire most citation.
These articles are considered
as representative of the corresponding research area.
Essentially, authors select keywords for their new articles either from the existing pool of keywords previously used or newly generated articles conjoined with the existing ones.
Therefore, few representative keywords having high degree centrality can always be found in KCN  ~\cite{choudhury2016time}. 
\begin{figure}[!h]
\begin{subfigure}{.20\textwidth}
    \includegraphics[width=1\textwidth]{{life2008}.pdf}
    \caption{$G_o$: 2008 (Life course)}
    \label{fig:2011oar}
\end{subfigure}
\begin{subfigure}{.35\textwidth}
    \includegraphics[width=1\textwidth]{{life2011}.pdf}
    \caption{$G_0$: 2011 (Life course)}
    \label{fig:2011oau}
\end{subfigure}
\begin{subfigure}{.44\textwidth}
    \includegraphics[width=1\textwidth]{{life2014}.pdf}
    \caption{$G_o$: 2014 (Life Course)}
    \label{fig:2011ode}
\end{subfigure}
\begin{subfigure}{.20\textwidth}
    \includegraphics[width=1\textwidth]{{endothelial2008}.pdf}
    \caption{$G_s$: 2008 (Endothelial dysfunction)}
    \label{fig:2014sar}
\end{subfigure}
\begin{subfigure}{.35\textwidth}
    \includegraphics[width=1\textwidth]{{endothelial2011}.pdf}
    \caption{$G_s$: 2011 (Endothelial dysfunction)}
    \label{fig:2014sau}
\end{subfigure}
\begin{subfigure}{.44\textwidth}
    \includegraphics[width=1\textwidth]{{endothelial2014}.pdf}
    \caption{$G_s$: 2014 (Endothelial dysfunction)}
    \label{fig:2014sde}
\end{subfigure}
\caption {\protect\raggedright Temporal evolution of associations between new and existing keywords demonstrated by two example keywords \textbf{\textit{Life course}} and \textbf{\textit{Endothelial dysfunction}} in $G_o$ and $G_s$ respectively. 
All network snapshots are timestamped and present the evolving connection patterns of the example keywords (green coloured) with the existing keywords (red and navy coloured) of the respective research domain. The red coloured keywords are the representative keywords of the research domain and acquire more connections over time.
The size of the node represents to the corresponding keyword's degree of connections. 
The thickness of the edges represents corresponding edge weights.}
\label{fig:knowledge_evolution}
\end{figure}
This phenomenon is demonstrated in Figure ~\ref{fig:knowledge_evolution} using two keywords \textbf{\textit{Life course}} and \textbf{\textit{Endothelial dysfunction}} (green coloured) from $G_o$ (a-c) and $G_s$ (d-f) respectively in three different times. 
In these figures, the red and navy coloured keywords are the existing keywords  where the former denote the representative keywords in the respective research domain.
The size variances of the keywords represent their degree of connections in the KCN of the corresponding time.
The edge thickness represents the edge weights.
From these network snapshots, it is observable that although new keywords emerge in association with less-acquainted (relatively low profile) keywords in the corresponding research area, however, gradually, they tend to co-appear with the representative keywords (e.g., cardiovascular disease in $G_o$ and metabolic syndrome in $G_s$).
It is observable that the example keywords form associations with existing keywords with relatively low degree.
However, over time, these example keywords get associated the high profile keywords within the research domain.
For example, the endothelial dysfunction for association with the keyword \textit{erectile dysfunction} in the year 2008.
In the year 2011, it form associations with the high degree keywords such as \textit{inflammation, hypoxia, metablic syndrome}.
In the year 2014, it acquire connections with more divergent high degree keywords of the domain (e.g., \textit{hypertension, sleep}.
% This denotes the fact that new keywords get endorsed by the representative keywords of a particular domain, an interesting observation yet to be observed in the citation network.
Consequently, the rich club phenomena is also evident in dynamic KCN analyses which can be captured by the degree centrality of the corresponding representative keywords.

Alongside the classical degree centrality measure, researchers attempted to define custom metrics to denote nodal importance. 
In one such study, Klimek et al.~\cite{klimek2016successful} developed a bipartite relations using term–document matrix and proposed a recursively defined document centrality measure to denote the importance of scientific documents.  
According to their assumption, a list of documents is considered central if these consume a large number of central terms those in turn also are consumed by a large number of central documents. Following their conceptualization of recursive document centrality measures, two recursive keyword centrality measures (i.e., $v^{au}_t$ and $v^{at}_t$) were developed for each keyword $v$ in each year $t$ of the training period.
The first centrality measure considers the keyword-author bipartite relations whereas the second, considered the keyword-article relation.
In case of the first bipartite relations, the intuition behind a keyword's importance is defined by the number of central authors who, in turn, also use a large number of central keywords. 

After the initial textual keyword and data processing, we filtered out those keywords appeared in only one article.
This category denotes the specialized keywords not related to the wide majority of the scientific articles. 
With the remaining number of keywords, we constructed a keyword-author adjacency matrix $M_{AxK}$ for each year $t$ in the training period. 
It is worth mentioning that we considered the first name and last name of the authors and manually verified with the affiliation information to perform author name disambiguation. 
Although the objective of this manual author name disambiguation was to find all publications that belong to a given author and distinguish them from publications of other authors who share the same name, however, exploration of other methods for the same purpose is left for future studies.
The adjacency matrix $M$ is a binary matrix of size $|A| \times |K|$ where $A$ and $K$ denote the set of authors and keywords respectively in year $t$. 
An entry in matrix $M$ is $1$ if the author $a \in A$ uses the keyword $k \in K$ in his/her article.
Starting with an example author $a_i$ in year $t$, for each keyword $k_i$ used by this author, we can reach all other authors who also used $k_i$ in their article. 
Iterating this procedure twice,  we reach all the authors in two-hop distance from $a_i$. 
These authors used keyword(s) that is also used by author(s) sharing some keywords with author $a_i$. 
Figure ~\ref{fig:origin} demonstrates the iteration procedure with some example keywords.
This measure accumulates the number of different paths available among authors through their keyword usages.
Higher number represents that the corresponding keyword is pervasive across the research domain and thus more central and familiar to the key authors.
To calculate recursive keyword centrality in this way, two vectors $\psi_k$ and $\psi_a$ are defined recursively:
\begin{equation}
\psi_k(n,t)=\frac{\sum_{a}M(t)\psi_a(n-1,t)}{\psi_k(0,t)} , \  
\psi_a(n,t)=\frac{\sum_{k}M(t)\psi_k(n-1,t)}{\psi_a(0,t)} 
\end{equation}
with $n$ represents the number of iterations as portrayed in Figure ~\ref{fig:origin}. $\psi_k(0,t)$  and $\psi_a(0,t)$ denote the initial conditions  as $\psi_k(0,t)=\sum_{a\in A} {M}(t)$ and $\psi_a(0,t)=\sum_{k \in K} {M}(t)$. 
The values of $\psi_k$ can have different interpretations.
\begin{figure}[!h]
    % \captionsetup{justification=centering}
    \includegraphics[width=.98\textwidth, height=9cm]{{original_centrality}.pdf}
    \caption{Computation of recursive keyword centrality measure using keyword-author relations. The computation is an iterative procedure that starts at an author, $a_0$. The first iteration counts the number of authors that used a keyword which is also used by $a_0$. Then this iteration continues until it reaches the terminating condition}
    \label{fig:origin}
\end{figure}
The initial condition $\psi_k(0,t)$ denotes the degree centrality of a keyword.
For different values of $n=1, 2, 3 ...$, values of $\psi_k$ assign weights to individual keywords considering the number of authors consuming them in their articles. 
Therefore, high values of $\psi_k$ corresponds to the keywords selected by a large number of authors those used large number of such keywords.
Conversely, low values represent the keywords` specificity and relevance to limited number of research issues. 
Similar observations are also true in case of $psi_a$.
The number of iteration converged  and found stable at $n=20$.
We also attempted higher value of $n$ however. found similar recursive centrality values returned by the algorithm.
Thus, for each year $t$ in the training period, we calculated a vector of z-score normalized recursive keyword centrality values $C^{au}_t$ by following the algorithm, from the keyword-author bipartite relations.
% The centrality measures were $z$-score normalized.
Likewise, another recursive keyword centrality measure $C^{at}_t$ was constructed from the keyword-article bipartite relations in each year $t$ during the training interval. 
In addition to these recursive centrality measures, to compare the results with a traditional centrality measure, we also calculated degree centrality values of keywords $C^d_t$, extracted from the unipartite keyword-keyword relations in KCN for each year $t$.
% Degree centrality values were extracted for prediction results comparison's sake.
Future studies can calculate other centrality values to compare the results further.



==> Other_pages/features.tex <==
\section {Predictive Features}
\setlabel{Predictive Features}{sec:link_feature}

% In this sections, we describe our feature construction procedures.
% Before describing some temporal and network characteristics of individual author selected keywords extracted from dynamic KCN, below are the description of some frequently used notations in Table \ref{notations}.


% \begin{table}[!h]
% \centering
% \begin{threeparttable}
% \caption{Frequently Used Notations}
% \label{notations}
% \begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}}ll}
% \toprule
% Notation    & Description \\
% \midrule
% ${k_{gp},k_p,k_c,k_g}$        & Four keyword types: {Grandparent, Parent, Children, Guest}                          \\
% % $C^{au},C^{at}$	& Vectors representing recursive keyword centrality measures computed from \\ & author-keyword and article-keyword bipartite relations 	\\
% $v^{au}_t,  v^{at}_t$    & Two variants of recursive centrality values for keyword $v$ at time $t$ (year) \\ & calculated from keyword-author and keyword-article bipartite relations\\
% $N^{au}_{t},N^{at}_{t}$ & Sets of top $N$ central keywords in year $t$ \\ & considering the bipartite network centrality measures\\

% % $t_s, t_f$ & Starting year and ending year of training time range $T$\\
% \bottomrule
% \end{tabular*}
% \end{threeparttable}
% \end{table}
% \subsection*{Keyword Characteristics}
% \setlabel{Keyword Characteristics}{sec:key_charac}
% In dynamic KCN, constructed from author selected keywords, the preferential attachment is a common phenomena of network evolution. 
% There are some domain representative keywords those define the thematic context of research under the corresponding.
% In additions to links among these domain-specific keywords, new keywords, defining emerging topics, also flock around these preponderant keywords.
% In course of time, emerging links emanate from these new keywords due to their increased familiarity and thus they become more prevalent.
% Consequently, due to their wide spread prevalence over time, they exert more network importance and accrue additional connections.
% Analogous to knowledge graph where new knowledge stem from existing and prevalent knowledge, dynamics of KCN resonates a genealogical graph of keywords.
% Genealogy is the study of family tree and a genealogy graph is used to present and depict the complex evolving relation originating from the ancestors.
% Dynamics of KCN simulate the knowledge graph where new knowledge stem from existing and prevalent knowledge.
% In the following subsections, we first describe two individual keyword (node-level) characteristics before employing them in the aggregated (edge-level) feature construction procedure.

 
% \begin{figure}[!h]
%     % \captionsetup{justification=centering}
%     \includegraphics[width=.98\textwidth, height=9cm]{{original_centrality}.pdf}
%     \caption{Computation of recursive keyword centrality measure using keyword-author relations. The computation is an iterative procedure that starts at an author, $a_0$. The first iteration counts the number of authors that used a keyword which is also used by $a_0$. Then this iteration continues until it reaches the terminating condition}
%     \label{fig:origin}
% \end{figure}
% \subsection {Keyword Features}
% \setlabel{Keyword Features}{sec:key_charac}
% In the following two subsections, we first describe individual keyword-specific characteristics before employing them in the feature construction procedure.

% \subsubsection {Recursive centrality}
% \setlabel{Recursive centrality}{sec:rec_centrality}
% Alongside classical centrality measures, researchers attempted to define custom metrics to denote nodal importance. 
% In one such study, Klimek et al.~\cite{klimek2016successful} developed a bipartite relations using term–document matrix and proposed a recursively defined document centrality measure to denote the importance of scientific documents.  
% According to their assumption, a list of documents is considered central if these consume a large number of terms those in turn also are consumed by a large number of central documents. Following their conceptualization of recursive document centrality measures, two recursive keyword centrality measures (i.e., $v^{au}_t$ and $v^{at}_t$) were developed for each keyword $v$ in each year $t$ of the training period.
% The first centrality measure considers the keyword-author bipartite relation whereas the second, following the metric proposed by ~\cite{klimek2016successful}, considers the keyword-article relation.
% In case of the keyword-author bipartite relations, the intuition behind a keyword's importance is defined by the number of central authors who, in turn, also use a large number of central keywords. 

% % \begin{figure}[!h]
% %     \centering
% %     \includegraphics[width=.97\textwidth]{{centrality}.pdf}
% %     \caption{Initial conditions and recursive keyword centrality measures from the matrix $M_{ka}$ representing keyword-author bipartite relations.}
% %     \label{fig:recursive}
% % \end{figure}

% After the initial textual keyword and data processing, we filtered out the most frequent common keywords not specific for scientific publications and those keywords appeared in only one article.
% The later category denotes the specialized keywords not related to the wide majority of the scientific articles. 
% With the remaining number of keywords, we constructed a keyword-author matrix $M_{ka}$ for each year $t$ in the training period. 
% It is worth mentioning that we considered the first name and last name of the authors and verified with the affiliation information to perform manual author name disambiguation. 
% Although the objective of this manual author name disambiguation was to find all publications that belong to a given author and distinguish them from publications of other authors who share the same name, however, exploration of other methods for the same purpose is left for future studies.
% The adjacency matrix $M$ is a binary matrix of size $|A| \times |K|$ where $A$ and $K$ denote the set of authors and keywords respectively in year $t$. 
% An entry in matrix $M_{ka}$ is $1$ if the author $a$ uses the keyword $k$ in his/her article.
% Starting with an example author $a_i$ in year $t$, for each keyword $k_i$ used by this author, we can reach all other authors who also used $k_i$ in their article. 
% Iterating this procedure twice,  we reach all the authors in two-hop distance from $a_i$. 
% These authors used keyword(s) that is also used by author(s) sharing some keywords with author $a_i$. 
% Figure ~\ref{fig:origin} demonstrates the iteration procedure with some example keywords.
% This measure accumulates the number of different paths available among authors through their keyword usages.
% Higher number represents that the corresponding keyword is pervasive across the research domain and thus more central and familiar to the key authors.
% To calculate recursive keyword centrality in this way, two vectors $\psi_k$ and $\psi_a$ are defined recursively:
% \begin{equation}
% \psi_k(n,t)=\frac{\sum_{a}M_{ka}(t)\psi_a(n-1,t)}{\psi_k(0,t)} , \  
% \psi_a(n,t)=\frac{\sum_{k}M_{ka}(t)\psi_k(n-1,t)}{\psi_a(0,t)} 
% \end{equation}
% with $n$ represents the number of iterations as portrayed in Figure ~\ref{fig:origin}. $\psi_k(0,t)$  and $\psi_a(0,t)$ denote the initial conditions  as $\psi_k(0,t)=\sum_a {M_{ka}}(t)$ and $\psi_a(0,t)=\sum_k {M_{ka}}(t)$. 
% % The computation process of initial conditions is visualized in Figure ~\ref{fig:recursive}. 
% The values of $\psi_k$ can have different interpretations.
% The initial condition $\psi_k(0,t)$ denotes the degree centrality of a keyword.
% For different values of $n=1, 2, 3 ...$, values of $\psi_k$ assign weights to individual keywords considering the number of authors consuming them in their articles. 
% Therefore, high values of $\psi_k$ corresponds to the keywords selected by a large number of authors those used large number of such keywords.
% Conversely, low values represent the keywords` specificity and relevance to limited number of research issues. 
% Similar observations are also true in case of $psi_a$.
% Following Klimek et al.~\cite{klimek2016successful}, we restricted the number of iteration at $n=20$ due to the convergence issue.
% We found that at higher values (i.e., $n>20$), the algorithm returns the same number as the centrality value.
% Thus, for each year $t$ in the training period, we calculated a vector of z-score normalized recursive keyword centrality values $C^{au}_t$ by following the algorithm, from the keyword-author bipartite relations.
% The centrality measures were $z$-score normalized.
% Likewise, another recursive keyword centrality measure $C^{at}_t$ was constructed from the keyword-article bipartite relations in each year $t$ during the training interval. 
% In addition to these recursive centrality measures, we also calculated degree centrality values of keywords $C^d_t$, extracted from the unipartite keyword-keyword relations in KCN for each year $t$.
% Degree centrality values were extracted for prediction results comparison's sake.

% \subsubsection {Genealogical typology}
% \setlabel{Genealogical typology}{sec:genealogy_typology}
% % \subsubsection*{Heredity score}
% % \setlabel{heredity score}{sec:heredity}	

% Preferential attachment is the most common phenomenon in keyword-based knowledge network ~\cite{choudhury2016time}. 
% Therefore in KCN, there exists a set of most central keywords which generally has greater influence over the structure of the network. 
% It was observed that other keywords generally tend to form relations by co-appearing with these rich keywords.
% To predict the future edges among keywords, we need to take this fact into consideration.
% % Besides, our experimental analysis showed that, a significant amount of keyword-keyword relations emerge and evolve around these central keywords.
% Our next keyword feature was constructed by capitalizing the idea of preferential attachment, however, in a different way.
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=.9\textwidth, height=8.5cm]{{heredity_build}.pdf}
%     \caption{Genealogical communities of keywords by considering a set of keywords with high recursive centrality values (i.e., $N^{au}_{t-1}$) computed from keyword-author bipartite relationships. Keywords with high centrality values at timestamp $t-1$ are designated as grandparents ($k_{gp}$ at timestamp $t$. Direct neighbours of these grandparents belong to parents ($k_p$) community, and two-hop neighbours are designated as children ($k_c$).Rest of the keywords are designated as guests ($k_g$).} 
%     \label{fig:heredity_build}
% \end{figure}
% We defined a keyword's genealogical score in each year that denotes it's current genealogical relation with previous year's central keywords. 
% The underlying objective here was to capture the evolution of keywords over the years and lineages to their ancestry. 
% Genealogy is the study of family tree and a genealogy graph is used to portray the complex evolving relation originating from the ancestors. 
% % As shown in Figure \ref{fig:genealogy}, the genealogy graph of node $x$ represents the node's relation with it's ancestors as well as descendants. 
% In the same way, we defined a keyword's role in a particular year $t$ based on it's relation with the central keywords from previous year $t-1$. 
% The centrality of keywords was measured by considering two recursive centrality measures and one degree centrality metrics defined above.
% This approach would label keywords according to the type of their family ancestral relationships (e.g., grandparents, parents, child or guest) and help us understanding the impact of these types in their co-occurrences.
% The computation of genealogical score is described below:
% In our dynamic KCN, we define four types of keywords, namely, grandparents $(k_{gp})$, parents $(k_p)$, children $(k_c)$ and guests $(k_g)$.
% If we consider labeling keywords in year $t$, then $k_{gp}$ keywords are the top-$N$ central keywords from year $t-1$. 
% Here, the word `central' higher values of three aforementioned centrality measures (i.e., two recursive and one degree centrality). 
% In other words, these are the most frequent and influential both in regards to the contents of metadata information (e.g.,author and article) and in forming relations with other keywords. 
% % The number $N$ was set to $20$ in our case, after testing the range of $(10-100)$. 
% In this way, we got two sets of top-$N$ central keyword values $N^{au}_{t-1},N^{at}_{t-1}$ based on our two recursive centrality measures (i.e., $C^{au}_{t-1}$, $C^{at}_{t-1}$). 
% The third heredity score was computed by considering the degree centrality values (i.e., $C^{d}_{t-1}$ of keywords from KCN. 
% These three sets can be used to generate three distinct heredity scores for each keywords. 

% Let $N^{au}_{t-1}$ denotes the top-$N$ central keywords identified by using keyword-author recursive centrality measure (i.e., $C^{au}_{t-1}$). 
% These $N$ keywords from year $t-1$ are labeled as grandparents $(k_{gp})$ in the year $t$.
% The set of other keywords having direct relations (i.e., an edge is observed between them) with $k_{gp}$ are labeled as parents $(k_p)$ in the year $t$. 
% Subsequently, children $(k_c)$ are the direct neighboring nodes of $k_p$ keywords but not $K_{gp}$. 
% Alternatively, $k_p$ keywords are considered as common neighbours between $k_{gp}$ and $k_c$. After defining these three communities of keywords (i.e. $k_{gp}, k_p, k_c$), we exclude them from the set of all keywords $(V_t)$ and label the rest as guests $(k_g)$.
% These guests are the keywords having maximum distance from the grandparents.
% In this way, we define the genealogical communities of all keywords appearing in a particular year. 
% % (as shown in Equation \eqref{eq:gp} - \eqref{eq:g}). 
% In our experiment, we use top-$N$ keywords from year $(t=0)$ (i.e., 2007) for the first training year $(t=1)$ (i.e., 2008), though this year $(t=0)$ is not included within our training period. 
% This fact was mentioned in the earlier section \ref{sec:data_acquisition}.
% \begin{figure}[!h]
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2008oar}.pdf}
% %     \caption{$G_o$: 2008 (article)}
% %     \label{fig:2008oar}
% % \end{subfigure}
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2008oau}.pdf}
% %     \caption{$G_o$: 2008 (author)}
% %     \label{fig:2008oau}
% % \end{subfigure}
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2008ode}.pdf}
% %     \caption{$G_o$: 2008 (degree)}
% %     \label{fig:2008ode}
% % \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{heredity/2011sar}.pdf}
%     \caption{$G_s$: 2011 (keyword-article)}
%     \label{fig:2011oar}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{heredity/2011sau}.pdf}
%     \caption{$G_s$: 2011 (keyword-author)}
%     \label{fig:2011oau}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{heredity/2011sde}.pdf}
%     \caption{$G_s$: 2011 (degree)}
%     \label{fig:2011ode}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{heredity/2014sar}.pdf}
%     \caption{$G_s$: 2014 (keyword-article)}
%     \label{fig:2014sar}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{heredity/2014sau}.pdf}
%     \caption{$G_s$: 2014 (keyword-author)}
%     \label{fig:2014sau}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{heredity/2014sde}.pdf}
%     \caption{$G_s$: 2014 (degree)}
%     \label{fig:2014sde}
% \end{subfigure}
% \caption {\protect\raggedright Temporal variations of genealogical traits demonstrated by keywords depending on the centrality measures used in $G_o$ dataset. 
% All network snapshots are timestamped including the centrality measure used to identify the genealogical traits.
% % For example, snapshot \ref{fig:2008oar} represents the sub-network of six keywords in $G_{o}$ for the year 2008 and the genealogical type of these keywords were computed by considering recursive centrality measures in keyword-article relations. 
% The color codes represent the genealogical communities of keywords: red (grandparent), green (parent) and blue (child). 
% The size of the node represents to the keyword's corresponding centrality measures. }
% \label{fig:h_variation}
% \end{figure}
% Next, we assign each keyword a score according to its genealogical relationship. 
% The successive order of keyword genealogical score is: $score(k_{gp}) >>score(k_p)>score(k_c)>score(k_g)$.
% Here, $k_{gp}$ are considered as the most influential keywords in the KCN of a year. 
% Despite the trivial quantity of these influential keywords, individually these were found to form most relations with others. 
% Consequently, we assigned them the highest score. 
% Scores for other three keyword types: $k_p$,$k_c$,$k_g$ are defined according to their distance from the grandparents $k_{gp}$. 
% Being the most distant ones, $k_g$ (guests) are assigned with lowest heredity score. 
% The process of labeling all keywords for a particular year $t$ using previous year's central keywords $(N^{au}_{t-1})$ and assigning the keyword's genealogy scores is depicted in figure \ref{fig:heredity_build}. 
% The relative size of each keyword trait in this figure represents the weight of the score (i.e. greater size for higher value). 
% Likewise, we computed two more sets of genealogical scores for each keyword using $N^{at}_{t-1}$ and $N^{d}_{t-1}$.

% Considering three sets of centrality measures of keywords (i.e., $v^{au}_t,  v^{at}_t$  and one degree centrality), a keyword having one genealogical trait(\eg, grandparent) in one set, might have different trait(\eg, parent) in another.This effectively means that if a keyword becomes grandparent by considering the $v^{au}_t$, it may not be necessarily true considering the other centrality measures (i.e., $v^{at}_t$ or degree centrality).
% Likewise, considering the same centrality measure, a keyword can belong to different genealogical typology in different year.
% % \begin{figure}[!h]
% % \begin{subfigure}{.24\textwidth}
% %     \includegraphics[width=0.83\textwidth]{{h-2010}.pdf}
% %     \caption{$G_s$: 2008-2010}
% %     \label{fig:h2010}
% % \end{subfigure}
% % % \begin{subfigure}{.25\textwidth}
% % %     \centering
% % %     \includegraphics[width=0.9\textwidth]{{h-2012}.pdf}
% % %     \caption{$G_s$: 2011-2012}
% % %     \label{fig:h2012}
% % % \end{subfigure}
% % \begin{subfigure}{.24\textwidth}
% %     \centering
% %     \includegraphics[width=0.83\textwidth]{{h-2014}.pdf}
% %     \caption{$G_s$: 2013-2014}
% %     \label{fig:h2014}
% % \end{subfigure}
% % \begin{subfigure}{.23\textwidth}
% %     \centering
% %     \includegraphics[width=0.85\textwidth]{{w-2012}.pdf}
% %     \caption{$G_o$: 2011-2012}
% %     \label{fig:w2012}
% % \end{subfigure}
% % \begin{subfigure}{.23\textwidth}
% %     \centering
% %     \includegraphics[width=0.85\textwidth]{{w-2014}.pdf}
% %     \caption{$G_o$: 2013-2014}
% %     \label{fig:w2014}
% % \end{subfigure}
% % % \begin{subfigure}{.3\textwidth}
% % %     \includegraphics[width=1\textwidth]{{w-2010}.pdf}
% % %     \caption{$G_o$: 2008-2010}
% % %     \label{fig:w2010}
% % % \end{subfigure}
% % % \hspace{5mm}
% % % \begin{subfigure}{.3\textwidth}
% % %     \centering
% % %     \includegraphics[width=1\textwidth]{{w-2012}.pdf}
% % %     \caption{$G_o$: 2011-2012}
% % %     \label{fig:w2012}
% % % \end{subfigure}
% % % \hspace{5mm}
% % % \begin{subfigure}{.3\textwidth}
% % %     \centering
% % %     \includegraphics[width=1\textwidth]{{w-2014}.pdf}
% % %     \caption{$G_o$: 2013-2014}
% % %     \label{fig:w2014}
% % % \end{subfigure}
% % \caption{Excerpts of network snapshots in $G_s$ dataset during \ref{fig:h2010} (2008-2010),  and \ref{fig:h2014} (2013-2014) presenting the neighbourhood of a central keyword  \textit{hypertension}. Excerpts of network snapshots in $G_o$ dataset during \ref{fig:w2012} (2011-2013), and \ref{fig:w2014} (2013-2014) for presenting the neighbourhood of keyword \textit{weight loss}. In these snapshots, color codes of nodes represent ancestry (family lineage) of keywords:grandparents (red), parents (green), children (blue) and guests (yellow). Relative sizes of both nodes and their label represent the recursive keyword centrality values extracted from  keyword-author bipartite relationships. The color codes of links represent three different years within each range except the duration 2013-2014. Green colored links appeared in the first year of the corresponding duration (\eg 2008 in \ref{fig:h2010}), orange represents links in the year 2009 and violet 2010. In \ref{fig:w2014} for the duration 2013-14, orange represents links in 2013 and violet represents links in 2014.}
% % \end{figure}
% % In the top row, 
% % \begin{figure}[!h]
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2008sar}.pdf}
% %     \caption{$G_s$: 2008 (article)}
% %     \label{fig:2008sar}
% % \end{subfigure}
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2008sau}.pdf}
% %     \caption{$G_s$: 2008 (author)}
% %     \label{fig:2008sau}
% % \end{subfigure}
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2008sde}.pdf}
% %     \caption{$G_s$: 2008 (degree)}
% %     \label{fig:2008sde}
% % \end{subfigure}
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2011sar}.pdf}
% %     \caption{$G_s$: 2011 (article)}
% %     \label{fig:2011sar}
% % \end{subfigure}
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2011sau}.pdf}
% %     \caption{$G_s$: 2011 (author)}
% %     \label{fig:2011sau}
% % \end{subfigure}
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2011sde}.pdf}
% %     \caption{$G_s$: 2011 (degree)}
% %     \label{fig:2011sde}
% % \end{subfigure}
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2014sar}.pdf}
% %     \caption{$G_s$: 2014 (article)}
% %     \label{fig:2014sar}
% % \end{subfigure}
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2014sau}.pdf}
% %     \caption{$G_s$: 2014 (author)}
% %     \label{fig:2014sau}
% % \end{subfigure}
% % \begin{subfigure}{.3\textwidth}
% %     \includegraphics[width=.8\textwidth]{{heredity/2014sde}.pdf}
% %     \caption{$G_s$: 2014 (degree)}
% %     \label{fig:2014sde}
% % \end{subfigure}
% % \caption{Keyword heredity variation ($G_{s}$)}
% % \label{fig:h_variation_apnea}
% % \end{figure}
% In Figure \ref{fig:h_variation}, a comparative representation of these variations of some keywords are presented in $G_s$ datasets.
% In this figure, top two rows present network snapshots of $G_o$ considering six keywords (i.e., \textit{\textbf{atherosclerosis, morbid obesity, diagnosis, excessive daytime sleepiness, behavior, and compliance}}).
% Surprisingly, these exists some commonality of keywords in both datasets since some of these keywords resemble to those in the obesity dataset.
% Since the commonality is out of the scope of this study, we leave it for future studies where domain experts can contribute towards literature-based discovery related to these two domains.
% The first row presents the network snapshots in the year 2011 and the second presents snapshots in the year 2014.
% % The third row represents three network snapshots cmprised of six keywords (i.e., \textit{\textbf{prevalence, myo-inositol, polycystic ovary syndrome, body weight, coronary artery disease and atherosclerosis}}) in $G_s$ in the year 2014.
% In each row, the left snapshot presents the genealogical typologies of keywords identified by considering the recursive centrality measures (i.e., $v^{at}_t$)  computed from keyword-article bipartite relations.
% Likewise, the snapshot in the middle column presents the genealogical typologies of keywords identified by considering the recursive centrality measures (.i.e., $v^{au}_t$) computed from keyword-author bipartite relations.
% The right column presents the similar, however, considering the keyword's degree centrality.
% Color codes represent different types of the keywords: grandparent (red), parent (green), and child (blue).  
% The sizes of the node and labels denote corresponding centrality values.
% % In the top row of this figure, ancestry labels of six keywords in $G_s$ are presented for seven years (2007-2014) duration of the training period. 
% It is observable that keywords can belong to different communities in different years by considering three different centrality measures used in this study.
% % It is noteworthy that we also collected data for the year 2007, however it was not included as a training year.
% % Keyword related information for the year 2007 was used to designate the keyword's traits for the year 2008.  
% % In this figure, keyword \textit{diagnosis} is grandparent according to \textit{author-keyword} $v^{au}_t$ recursive centrality measure and \textit{degree} $v^{d}_t$ centrality but parent according to the \textit{article-keyword} $v^{ar}_t$ centrality values. 
% % In case of \textit{morbid obesity} in the year 2012, it is labeled as guest by the $v^{au}_t$ centrality values, grandparent by the $v^{aa}_t$, and child according to $v^{d}_t$ respectively. 
% % Being grandparent according to $v^{ar}_t$ signifies that it was used a large number of times in those articles, which in turn use large number of central keywords. 
% % Conversely, being guest by $v^{au}_t$ means, it failed to gain attention from authors who used large number of central keywords. 
% % In addition, it was considered as child keyword in regards to degree centrality as it found as two-hop neighbor from most dominant keywords of the previous year.
% % Similar observations are presented for $G_o$ dataset in the bottom row of the figure. 
% % Due to the high density of this dataset in comparison to $G_s$ dataset, the rate of such variation in keyword's traits is limited. The grandparent keywords remain in the range of parenthood at most according to different centrality measures. 
% Consider the genealogical types of the keyword \textit{diagnosis}.
% In the year 2011, it is designated as grandparent by considering the recursive centrality measure from keyword-article relations, whereas considering the same centrality measure, it belongs to `parent' community in 2014.
% Surprisingly, the later is also true when recursive centrality measure from the keyword-author relations was considered in the yer 2011.
% Similar observations are evident in case of the keyword \textit{behaviour}
% % In this figure, keyword \textit{myo-inositol} did not appear in the year 2009 and 2014.
% % This irregularity also justifies it's genealogical typology. 
% % Apart from the exception in 2012, it always appeared as a guest keyword mostly. 
% % In 2012, active presence of this keyword was observed where it appeared as parent by considering all three types of centrality values. 
% There are other domain-specific keywords (\eg   \textit{sleep}, \textit{apnea},\textit{ obesity}) those were found as grandparents in all variants because of their relevancy to the domain.

% \subsubsection {Citation score}
% Scientific authors publish articles as part of communicating their research findings and also seek to ensure maximum possible research impact, reflect their talents and create new opportunities.
% Consequently, articles would draw attention of their fellow researchers and receive many citations if they cover important research topics and/or are relevant and useful ~\cite{garfield2006history}.
% Therefore, the scientific communities have widely adopted citation counts as the principal representative factor of the impact of scientific research. 
% In addition, these counts are used as an indication of an individual’s research productivity ~\cite{duffy2011research}.
% Considering their importance, in this study, we also utilized the aggregation of citation counts of papers.
% Thus a keyword's citation count represents the total number of citation counts of the articles where the corresponding keyword appeared in each year. 
% To make use of frequent appearances and influential nature of keywords, we considered their yearly citation count in our dynamic link prediction task.

% \subsection {Aggregated Features}
% \setlabel{Aggregated Features}{sec:aggregated_feature}
% In the aforementioned section, we have identified 
% individual attributes of keywords that can  provide helpful clues for link
% prediction. 
% Since, these attributes only pertain to one
% keyword in KCN, some aggregation functions
% need to be used to combine the attribute values of the corresponding keywords in a keyword-pair.
% To illustrate further, if either(or both) of the
% keywords are prolific or belong to the same community, it is more likely that they will co-occur.
% Before aggregation, the individual measure denotes the proliferation rate of individual keyword,  its community membership, temporal activeness (number of co-occurrences), or temporal importance.
% % how prolific a particular scientist is and the corresponding individual feature is the number of different areas
% % (s)he has worked on. 
% Combination of these individual features yields the aggregated features that is meaningful
% for the pair of keywords for dynamic link prediction.
% In this study's context, we assume that the higher the aggregated feature value, the more likely that two keywords will co-occur.

% \subsubsection {Temporal heredity score}
% \setlabel{Temporal heredity score}{sec:heredity}	

% This is the first feature we computed for each non-connected keyword-pairs for the link prediction purpose.
% The objective of this feature was to capitalize on the origin information (congenital traits) and current activeness (keyword's centrality measures) of both ends of every link.  
% In the above sections, we have defined few important characteristics of keywords by leveraging the temporal keyword co-occurrences networks and historical family lineage. 
% These are: firstly,  \ref{sec:rec_centrality} measures and secondly, their \ref{sec:genealogy_typology}.
% % We have defined two types of recursive centrality measures: $v^{au}_t$ was computed from keyword-author relations and $v^{at}_t$ was computed from article-keyword relations for each keyword $v$ at time $t$. 
% % The third type of centrality measure $v^{d}_t$ was defined based on keyword's temporal degree centrality.
% % In regards to genealogical traits, we categorized keywords into grandparents, parents, children and guests.
% To develop features, characterising keyword-pairs, we combined and aggregated these keyword features.
% For each type of centrality measure, we multiplied keywords corresponding centrality values with its genealogical typology (i.e., community) score.
% % To be more precise, considering $v^{au}_{t-1}$ which is the recursive centrality value of keyword $v$ extracted from the keyword-author relations at timestamp $t-1$, we first determined its community score (grandparent/parent/child/guest) at time $t$.
% % Then the aggregated value for keyword $v$ was computed by multiplying it's community score with $v^{au}_t$, its recursive centrality score.
% Chenhao Tan \citep{genealogy} investigated how the origin of a community connects to its future growth and how the history of the early members allows us to understand the emergence of communities (i.e., tracing the origin of a community)
% By demonstrating the fact that strong parent connections are important for future community growth, the author believed that the emerging process of a community is analogous to complex contagion that requires dense connections between
% early adopters.
% In our case the early adopters are the members of the grandparent and parent communities.
% Consequently, the aggregated feature scores should have their community scores augmented.
% Therefore, for each year in the training period, we first multiply individual keyword's community score which denotes its relation with previous year's central keyword (i.e., keyword's heredity) with its corresponding centrality value which was used to determine its community membership.
% This determines the heredity score of individual keywords in each training year.
% % The intuition behind this is to exploit the keyword's current community status by using information of its origin (i.e., relation with previous year's central keyword - keyword's heredity) and its current activity/importance (\eg, centrality values).
% % This can be beneficial in predicting its future status \citep{genealogy}.
% Finally, by following Choudhury \& Uddin \citep{choudhury2016time}, for each keyword-pair, the feature value of temporal heredity score was computed by summing their aggregated heredity scores for each year $t$.
% The construction of our first keyword-keyword feature value at each timestamp $t$ in the training period, known as temporal heredity score between keyword $a$ and $b$ can be summarized as:
% % Therefore, at timestamp $t$, if $v^{au}_t$ is the author-keyword recursive centrality value of keyword $v$ and $v^{g_{au}}_t$ denotes its congenital trait score by considering the same recursive centrality measure, we computed our first feature value for keyword-pair $(u,v)$: 
% \begin{align}
% \begin{split}
% &score^H_t(a,b) = c^{au}_t(a)\cdot v^{au}_t(a) + c^{au}_t(b)\cdot v^{au}_t(b)
% \end{split}
% \label{eq:typology}
% \end{align}
% where $c^{au}_t(a)$ and $v^{au}_t(a)$ denote the genealogical typology (i.e., community) \ref{sec:genealogy_typology} and the corresponding centrality scores \ref{sec:rec_centrality}. In this way we built time series of temporal heredity scores for each instance of non-connected keyword pair of the classification dataset.


% % \ncnote{-----\\}
% % Following this, for each non-connected keyword-pair in each year of the training period, we constructed a time series of this feature value along with it's node level features which were input to the deep learning framework. For example, a 2D feature matrix of size $|T| \times |F|$ is generated for keyword pair $(u,v)$. Here, $T$ denotes the set of training years, whereas, $F$ is the set of related node-level and edge-level features for each training year. In other words, $F={score^G_t(u,v), k^{au}_t(u), c^{au}_t(v), k^{au}_t(v)}$ for the calculated heredity score in \eqref{eq:typology}. To train the LSTM network, these time-series are given as training inputs while, corresponding feature values for test year edges are given as target outputs. After the training phase, we can get the forecasted feature values for a test year edge using this model by providing it's training period feature values.

% \subsubsection {Citation-weighted Recency}
% \setlabel{Citation-weighted Recency}{sec:cit_recency}	
% % Scientific authors publish articles as part of communicating their research findings and also seek to ensure maximum possible research impact, reflect their talents and create new opportunities.
% % Consequently, articles would draw attention of their fellow researchers and receive many citations if they cover important research topics and/or are relevant and useful ~\cite{garfield2006history}.
% % Therefore, the scientific communities have widely adopted citation counts as the principal representative factor of the impact of scientific research. 
% % In addition, these counts are used as an indication of an individual’s research productivity ~\cite{duffy2011research}.
% % Considering their importance, in this study, we also utilized the aggregation of citation counts of papers.
% % Thus a keyword's citation count represents the total number of citation counts of the articles where the corresponding keyword appeared in each year. 
% % To make use of frequent appearances and influential nature of keywords, we considered their yearly citation count in our dynamic link prediction task.
% An individual keyword's citation count represent its influence factor over other keywords.
% However, domain-specific and old keywords can achieve higher citation counts then the others.
% Relative influence factor should also be brought into consideration.
% For example, old keywords accumulate more citation over time then new keywords.
% In contrast, some new keywords can gain significance quickly and acquire relatively high citation then other insignificant but old keywords.
% Therefore, we considered the temporal factors of keyword's appearances such as current or distant appearances over time. 
% Considering our training period (\eg, 2008-2014), an article published in 2008 gets more time to be cited than a article published in 2014. 
% Despite, the later one carries more impact, the former one is more weighted based on the numbers. 
% Further, training year closer to test period is more significant than earlier years since recently co-appeared keywords are more likely to come together in near future, a fact known as `recency' in link prediction task ~\cite{yang2012predicting}.

% Considering the aforementioned facts on temporal significance and citation count, we constructed our second feature for keyword pairs by accommodating both temporal recency and citation counts over time.
% % and In this feature, we also take attempts to improve the quality of data.
% % In other words, we make use of the partial available information to fill missing values for keywords when we found those absent in a particular year of training.  
% % Consider keyword $k$ appears in articles $A={a_1, a_2,\cdots,a_n}$ in training year $t$. If $cite(a_n)$ is the citation count of article $a_n$, then the total  citation count of keyword $k$ in year $t$ can be written as $c^k_t$. 
% % \begin{align}
% % &c^k_t=\Sigma_{n=1}^{|A|}cite(a_{n})\\ 
% % \begin{split}
% % &\text{where,} \\
% % &A=\text{set of articles where keyword $k$ appears and $a_n \in A$}
% % \end{split}
% % \end{align}
% Since citation count and temporal recency are applicable to individual keywords, it requires to aggregate these counts for keyword-pairs.
% % As this is the node level information of keyword $k$, we need to aggregate it in edge-level to use in our setup. 
% For each non-connected keyword-pair in year $t$, we aggregate their total citation counts. 
% Further, we assign temporal recency score depending on the appearances of both keywords in a particular year.
% The current their appearances are or alternatively, the closer their appearances towards the test duration, the higher the recency score.
% Considering the keyword-pair $(a,b)$, let  $t$ denotes the training year $t \in [1, 2, 3, ... T]$, $h^u_t$ and $h^v_t$ denote the total number of citation counts of the articles in year $t$ where keywords $a$ and $b$ appears respectively, then the weighted-citation recency is calculated as follows:

% \begin{align}
% \begin{split}
% &score^W_t(a,b) =  (h^a_t + h^b_t) \cdot \gamma t 
% \end{split}
% \label{eq:recency}
% \end{align}
% Here, $\gamma$ amplifies the recency effect and its value is two if both keywords in a keyword-pair appear in a year, one if either of the keyword appear, or zero (0) otherwise. 
% $h^a_t$  will be assigned zero value if keyword $a$ does not appear in an article that received any citation.
% However, the feature value will be augmented depending on the current appearances of the keywords (i.e., multiplied by value of $t$). 
% The assumption here is that, keywords having high citation in the recent years will have high probability to appear together since they represent the recent trends.

% % \ncnote{------\\}
% % Calculated edge feature in \eqref{eq:recency} along with it's node level features are given as LSTM training input following the approach described in previous section. Here, the feature set $F$ for year $t$ and keyword pair $(u,v)$ includes $^W_t(u,v), h^u_t, h^v_t$. Then using the trained model, we can get the forecasted feature values for test year, that will be further used for the link classification task.


==> Other_pages/keyword_feature.tex <==
\subsection {Keyword Features}
\setlabel{Keyword Features}{sec:key_charac}
Considering the temporal dynamics of keywords in dynamic KCN, evolutionary aspects of network influence, and traces of family lineage, we first identified some important characteristics of individual author selected keyword and classify them into different groups (i.e., communities). 

% \subsubsection {Recursive centrality}
% \setlabel{Recursive centrality}{sec:rec_centrality}
% Alongside classical centrality measures, researchers attempted to define custom metrics to denote nodal importance. 
% In one such study, Klimek et al.~\cite{klimek2016successful} developed a bipartite relations using term–document matrix and proposed a recursively defined document centrality measure to denote the importance of scientific documents.  
% According to their assumption, a list of documents is considered central if these consume a large number of central terms those in turn also are consumed by a large number of central documents. Following their conceptualization of recursive document centrality measures, two recursive keyword centrality measures (i.e., $v^{au}_t$ and $v^{at}_t$) were developed for each keyword $v$ in each year $t$ of the training period.
% The first centrality measure considers the keyword-author bipartite relations whereas the second, considered the keyword-article relation.
% In case of the first bipartite relations, the intuition behind a keyword's importance is defined by the number of central authors who, in turn, also use a large number of central keywords. 

% After the initial textual keyword and data processing, we filtered out those keywords appeared in only one article.
% This category denotes the specialized keywords not related to the wide majority of the scientific articles. 
% With the remaining number of keywords, we constructed a keyword-author adjacency matrix $M_{AxK}$ for each year $t$ in the training period. 
% It is worth mentioning that we considered the first name and last name of the authors and manually verified with the affiliation information to perform author name disambiguation. 
% Although the objective of this manual author name disambiguation was to find all publications that belong to a given author and distinguish them from publications of other authors who share the same name, however, exploration of other methods for the same purpose is left for future studies.
% The adjacency matrix $M$ is a binary matrix of size $|A| \times |K|$ where $A$ and $K$ denote the set of authors and keywords respectively in year $t$. 
% An entry in matrix $M$ is $1$ if the author $a \in A$ uses the keyword $k \in K$ in his/her article.
% Starting with an example author $a_i$ in year $t$, for each keyword $k_i$ used by this author, we can reach all other authors who also used $k_i$ in their article. 
% Iterating this procedure twice,  we reach all the authors in two-hop distance from $a_i$. 
% These authors used keyword(s) that is also used by author(s) sharing some keywords with author $a_i$. 
% Figure ~\ref{fig:origin} demonstrates the iteration procedure with some example keywords.
% This measure accumulates the number of different paths available among authors through their keyword usages.
% Higher number represents that the corresponding keyword is pervasive across the research domain and thus more central and familiar to the key authors.
% To calculate recursive keyword centrality in this way, two vectors $\psi_k$ and $\psi_a$ are defined recursively:
% \begin{equation}
% \psi_k(n,t)=\frac{\sum_{a}M(t)\psi_a(n-1,t)}{\psi_k(0,t)} , \  
% \psi_a(n,t)=\frac{\sum_{k}M(t)\psi_k(n-1,t)}{\psi_a(0,t)} 
% \end{equation}
% with $n$ represents the number of iterations as portrayed in Figure ~\ref{fig:origin}. $\psi_k(0,t)$  and $\psi_a(0,t)$ denote the initial conditions  as $\psi_k(0,t)=\sum_{a\in A} {M}(t)$ and $\psi_a(0,t)=\sum_{k \in K} {M}(t)$. 
% The values of $\psi_k$ can have different interpretations.
% The initial condition $\psi_k(0,t)$ denotes the degree centrality of a keyword.
% For different values of $n=1, 2, 3 ...$, values of $\psi_k$ assign weights to individual keywords considering the number of authors consuming them in their articles. 
% Therefore, high values of $\psi_k$ corresponds to the keywords selected by a large number of authors those used large number of such keywords.
% Conversely, low values represent the keywords` specificity and relevance to limited number of research issues. 
% Similar observations are also true in case of $psi_a$.
% The number of iteration converged  and found stable at $n=20$.
% We also attempted higher value of $n$ however. found similar recursive centrality values returned by the algorithm.
% Thus, for each year $t$ in the training period, we calculated a vector of z-score normalized recursive keyword centrality values $C^{au}_t$ by following the algorithm, from the keyword-author bipartite relations.
% % The centrality measures were $z$-score normalized.
% Likewise, another recursive keyword centrality measure $C^{at}_t$ was constructed from the keyword-article bipartite relations in each year $t$ during the training interval. 
% In addition to these recursive centrality measures, to compare the results with a traditional centrality measure, we also calculated degree centrality values of keywords $C^d_t$, extracted from the unipartite keyword-keyword relations in KCN for each year $t$.
% % Degree centrality values were extracted for prediction results comparison's sake.
% Future studies can calculate other centrality values to compare the results further.
% \subsubsection {Genealogical typology}
% \setlabel{Genealogical typology}{sec:genealogy_typology}

% Preferential attachment is the most common phenomenon in keyword-based knowledge network ~\cite{choudhury2016time}. 
% Therefore in KCN, there exists a set of most central keywords which generally has greater influence over the structure of the network. 
% It was observed that other keywords generally tend to form relations by co-appearing with these rich keywords.
% To predict the future connections between keywords, we need to take this fact into consideration.
% Our next keyword feature was constructed by capitalizing the idea of preferential attachment, but in a different way.
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=.9\textwidth, height=8.5cm]{{heredity_build}.pdf}
%     \caption{Genealogical communities of keywords by considering a set of keywords with high recursive centrality values (i.e., $N^{au}_{t-1}$) computed from keyword-author bipartite relationships. Keywords with high centrality values at timestamp $t-1$ are designated as grandparents ($k_{gp}$ at timestamp $t$. Direct neighbours of these grandparents belong to parents ($k_p$) community, and two-hop neighbours are designated as children ($k_c$).Rest of the keywords are designated as guests ($k_g$).} 
%     \label{fig:heredity_build}
% \end{figure}
% We defined a keyword's genealogical community score in each year that denotes it's current ancestral relation with previous year's central keywords. 
% The underlying objective here was to capture the evolution of keywords over the years and lineages to their ancestry. 
% Genealogy is the study of family tree and a genealogy graph is used to portray the complex evolving relation originating from the ancestors. 
% In the same way, we defined a keyword's family relationship in a particular year $t$ based on it's relation with the central keywords from previous year $t-1$. 
% The centrality of keywords was measured by considering two recursive centrality measures and one degree centrality metrics defined above.
% This approach would label keywords according to the type of their family ancestral relationships (e.g., grandparents, parents, child or guest) and help us understanding the impact of these types in their co-occurrences.
% The computation of genealogical community score is described below:

% In our dynamic KCN, we defined four types of communities for keywords, namely, grandparents $(k_{gp})$, parents $(k_p)$, children $(k_c)$ and guests $(k_g)$.
% Firstly, we defined the grandparents.
% If we consider identifying community membership of keywords in year $t$, then grandparents $k_{gp}$ keywords are the top-$N$ central keywords from year $t-1$. 
% Here, the word `central' denotes higher values of a chosen centrality measure from the three aforementioned centrality measures (i.e., two recursive and one degree centrality). 
% In other words, these are the most frequent and influential keywords both in regards to the contents of metadata information (e.g.,author and article) and in forming relations with other keywords. 
% We experimented with the number of grandparents ranging from $10-200$ by considering two recursive centrality meausres.
% Interestingly, we found that having $N\geqslant20$  grandparents in each year does not change the prediction performance significantly in both datasets.
% Therefore, we designated the top $20$ keywords as grandparents by considering two recursive centrality measures. 
% In the result section, we present the recursive centrality values  $v^{au}_t$ of keywords belonging to four communities and participating in the edges during the test year (2015).
% The clusters of all keywords will be evident in support of this choice.
% Replicating the same decision choice, we also keep the number of grandparents at $N=20$ by considering the degree centrality values of the keywords.
% In this way, we got three sets of top-$20$ central keywords  based on our three recursive centrality measures (i.e., $C^{au}_{t-1}$, $C^{at}_{t-1}$, and $C^{d}_{t-1}$). 
% Secondly, we define the parents, children and guests.
% % Let $N^{au}_{t-1}$ denotes the top-$N$ central keywords identified by using keyword-author recursive centrality measure (i.e., $C^{au}_{t-1}$). 
% % These $N$ keywords from year $t-1$ are labeled as grandparents $(k_{gp})$ in the year $t$.
% Keywords having direct relations (i.e., an edge is observed between them) with $k_{gp}$ are labeled as parents $(k_p)$ in the year $t$. 
% Subsequently, children $(k_c)$ are the direct neighboring nodes of $k_p$ keywords but not $K_{gp}$. 
% Alternatively, $k_p$ keywords are considered as common neighbours between $k_{gp}$ and $k_c$. 
% After defining these three communities of keywords (i.e. $k_{gp}, k_p, k_c$), we exclude them from the set of all keywords $(V_t)$.
% Rest of unlabeled keywords are designated as guests $(k_g)$.
% These guests keywords had maximum distance from the grandparents.
% In this way, we defined the genealogical communities of all keywords appearing in a particular year. 
% % (as shown in Equation \eqref{eq:gp} - \eqref{eq:g}). 
% In our experiment, we use top-$20$ keywords from year $(t=0)$ (i.e., 2007) for the first training year $(t=1)$ (i.e., 2008), though this year $(t=0)$ is not included within our training period. 
% This fact was mentioned in the earlier section \ref{sec:data_acquisition}.
% \begin{figure}[!h]
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{2011sar}.pdf}
%     \caption{$G_s$: 2011 (keyword-article)}
%     \label{fig:2011oar}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{2011sau}.pdf}
%     \caption{$G_s$: 2011 (keyword-author)}
%     \label{fig:2011oau}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{2011sde}.pdf}
%     \caption{$G_s$: 2011 (degree)}
%     \label{fig:2011ode}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{2014sar}.pdf}
%     \caption{$G_s$: 2014 (keyword-article)}
%     \label{fig:2014sar}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{2014sau}.pdf}
%     \caption{$G_s$: 2014 (keyword-author)}
%     \label{fig:2014sau}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1\textwidth]{{2014sde}.pdf}
%     \caption{$G_s$: 2014 (degree)}
%     \label{fig:2014sde}
% \end{subfigure}
% \caption {\protect\raggedright Temporal variations of genealogical traits demonstrated by keywords depending on the centrality measures used in $G_o$ dataset. 
% All network snapshots are timestamped including the centrality measure used to identify the genealogical traits.
% The color codes represent the genealogical communities of keywords: red (grandparent), green (parent) and blue (child). 
% The size of the node represents to the keyword's corresponding centrality measures. }
% \label{fig:h_variation}
% \end{figure}
% Next, we assign each keyword a score according to its ancestral relationship or genealogical community. 
% The successive order of keyword's genealogical community score is: $score(k_{gp}) >> score(k_p)> score(k_c)> score(k_g)$.
% Here, $k_{gp}$ keywords are considered as the most influential keywords in the KCN of a particular year. 
% Although, this does not necessarily mean that grandparents will have most of the connections since top central keywords in the previous year will not necessarily be on the top in the current year. 
% % Despite the trivial quantity of these influential keywords every year, individually these were found to form most relations with others. 
% However, being most influential in the previous year, we assigned them the highest score in the current year. 
% Scores for the other three keyword types: $k_p$,$k_c$,$k_g$ were defined according to their distance from the grandparents $k_{gp}$. 
% Being the most distant ones, $k_g$ (guests) are assigned with lowest community score. 
% The process of labeling all keywords for a particular year $t$ using previous year's central keywords and assigning the keyword's genealogical community scores is depicted in figure \ref{fig:heredity_build}. 
% The relative size of each keyword in this figure represents the weight of the score (i.e. greater size for higher value). 
% % Likewise, we computed two more sets of genealogical scores for each keyword using $N^{at}_{t-1}$ and $N^{d}_{t-1}$.
% In this figure, $N^{au}_{t-1}$ denotes the set of ton-$N$ central keywords by considering recursive centrality values $v^{au}_t$ extracted from keyword-author relations.

% Considering three sets of centrality measures of keywords (i.e., $v^{au}_t,  v^{at}_t$  and $v^{d}_t$), a keyword belonging to one genealogical community (\eg, grandparent) in one set, might belong to different community(\eg, parent) in another.
% This effectively means that if a keyword becomes grandparent by considering the $v^{au}_t$, it may not necessarily be true by considering the other centrality measures (i.e., $v^{at}_t$ or degree centrality).
% Likewise, considering the same centrality measure, a keyword can belong to different genealogical typology in different year.
% In Figure \ref{fig:h_variation}, a comparative representation of these variations of some keywords are presented in $G_s$ datasets.
% In this figure, top two rows present network snapshots in $G_s$ considering six keywords (i.e., \textit{\textbf{atherosclerosis, morbid obesity, diagnosis, excessive daytime sleepiness, behavior, and compliance}}).
% It is evident that there exists some commonality of keywords in both datasets since some of these keywords resemble to those in the $G_o$ dataset.
% Since the commonality is out of the scope of this study, we leave it for future studies where domain experts can contribute towards literature based discovery related to these two domains together.
% The first row in this figure presents the network snapshots in the year 2011 and the second presents snapshots in the year 2014.
% In each row, the left snapshots present the genealogical typologies (i.e., communities) of keywords identified by considering the recursive centrality measures (i.e., $v^{at}_t$)  computed from keyword-article bipartite relations.
% The snapshots in the middle column presents the genealogical typologies of keywords identified by considering the recursive centrality measures (.i.e., $v^{au}_t$) computed from keyword-author bipartite relations.
% The right column presents the similar, however, considering the keyword's degree centrality.
% Color codes represent different types of the keywords: grandparent (red), parent (green), and child (blue).  
% The sizes of the node and labels denote corresponding centrality values.
% It is observable that keywords can belong to different communities in different years by considering different centrality measures used in this study.
% Consider the genealogical types of the keyword \textit{diagnosis}.
% In the year 2011, it is designated as `grandparent' by considering  $v^{at}_t$, whereas considering the same centrality measure, it belongs to `parent' community in 2014.
% Surprisingly, the later is also true (`parent') when recursive centrality measure $v^{au}_t$ was considered in the year 2011.
% Similar observations are evident in case of the keyword \textit{behaviour}
% There are some domain-specific keywords (\eg   \textit{sleep}, \textit{apnea},\textit{ obesity}) those were found as `grandparents' in all variants because of their relevancy to the domain.

\subsubsection {Citation score}
Scientific authors publish articles as part of communicating their research findings and also seek to ensure maximum possible research impact, reflect their talents and create new opportunities.
Consequently, articles would draw attention of their fellow researchers and receive many citations if they cover important research topics and/or are relevant and useful ~\cite{garfield2006history}.
Therefore, the scientific communities have widely adopted citation counts as the principal representative factor of the impact of scientific research. 
In addition, these counts are used as an indication of an individual’s research productivity ~\cite{duffy2011research}.
Considering their importance, in this study, we also utilized the citation counts of articles.
Thus a keyword's citation count represents the total number of citation counts of the articles where the corresponding keyword appeared in each year. 
To make use of frequent appearances and influential nature of keywords, we considered a relative score of their yearly citation count in our dynamic link prediction task.


==> Other_pages/recursive_centrality.tex <==
\subsection {Preferential Attachment and Recursive Centrality}
\setlabel{Recursive centrality}{sec:rec_centrality}
The generation of author selected keywords is governed by the inherent rules of scholarly communication which is also known as preferential attachment ~\cite{zhao2018ranking}.
In citation-based scholarly communication, few articles within a research area will draw most attention and subsequently acquire most citation.
These articles are considered
as representative of the corresponding research area.
Essentially, authors select keywords for their new articles either from the existing pool of keywords previously used or newly generated articles conjoined with the existing ones.
Therefore, few representative keywords having high degree centrality can always be found in KCN  ~\cite{choudhury2016time}. 
\begin{figure}[!h]
\begin{subfigure}{.20\textwidth}
    \includegraphics[width=1\textwidth]{{life2008}.pdf}
    \caption{$G_o$: 2008 (Life course)}
    \label{fig:2011oar}
\end{subfigure}
\begin{subfigure}{.35\textwidth}
    \includegraphics[width=1\textwidth]{{life2011}.pdf}
    \caption{$G_0$: 2011 (Life course)}
    \label{fig:2011oau}
\end{subfigure}
\begin{subfigure}{.44\textwidth}
    \includegraphics[width=1\textwidth]{{life2014}.pdf}
    \caption{$G_o$: 2014 (Life Course)}
    \label{fig:2011ode}
\end{subfigure}
\begin{subfigure}{.20\textwidth}
    \includegraphics[width=1\textwidth]{{endothelial2008}.pdf}
    \caption{$G_s$: 2008 (Endothelial dysfunction)}
    \label{fig:2014sar}
\end{subfigure}
\begin{subfigure}{.35\textwidth}
    \includegraphics[width=1\textwidth]{{endothelial2011}.pdf}
    \caption{$G_s$: 2011 (Endothelial dysfunction)}
    \label{fig:2014sau}
\end{subfigure}
\begin{subfigure}{.44\textwidth}
    \includegraphics[width=1\textwidth]{{endothelial2014}.pdf}
    \caption{$G_s$: 2014 (Endothelial dysfunction)}
    \label{fig:2014sde}
\end{subfigure}
\caption {\protect\raggedright Temporal evolution of associations between new and existing keywords demonstrated by two example keywords \textbf{\textit{Life course}} and \textbf{\textit{Endothelial dysfunction}} in $G_o$ and $G_s$ respectively. 
All network snapshots are timestamped and present the evolving connection patterns of the example keywords (green coloured) with the existing keywords (red and navy coloured) of the respective research domain. The red coloured keywords are the representative keywords of the research domain and acquire more connections over time.
The size of the node represents to the corresponding keyword's degree of connections. 
The thickness of the edges represents corresponding edge weights.}
\label{fig:knowledge_evolution}
\end{figure}
This phenomenon is demonstrated in Figure ~\ref{fig:knowledge_evolution} using two keywords \textbf{\textit{Life course}} and \textbf{\textit{Endothelial dysfunction}} (green coloured) from $G_o$ (a-c) and $G_s$ (d-f) respectively in three different times. 
In these figures, the red and navy coloured keywords are the existing keywords  where the former denote the representative keywords in the respective research domain.
The size variances of the keywords represent their degree of connections in the KCN of the corresponding time.
The edge thickness represents the edge weights.
From these network snapshots, it is observable that although new keywords emerge in association with less-acquainted (relatively low profile) keywords in the corresponding research area, however, gradually, they tend to co-appear with the representative keywords (e.g., cardiovascular disease in $G_o$ and metabolic syndrome in $G_s$).
It is observable that the example keywords form associations with existing keywords with relatively low degree.
However, over time, these example keywords get associated the high profile keywords within the research domain.
For example, the endothelial dysfunction for association with the keyword \textit{erectile dysfunction} in the year 2008.
In the year 2011, it form associations with the high degree keywords such as \textit{inflammation, hypoxia, metablic syndrome}.
In the year 2014, it acquire connections with more divergent high degree keywords of the domain (e.g., \textit{hypertension, sleep}.
% This denotes the fact that new keywords get endorsed by the representative keywords of a particular domain, an interesting observation yet to be observed in the citation network.
Consequently, the rich club phenomena is also evident in dynamic KCN analyses which can be captured by the degree centrality of the corresponding representative keywords.

Alongside the classical degree centrality measure, researchers attempted to define custom metrics to denote nodal importance. 
In one such study, Klimek et al.~\cite{klimek2016successful} developed a bipartite relations using term–document matrix and proposed a recursively defined document centrality measure to denote the importance of scientific documents.  
According to their assumption, a list of documents is considered central if these consume a large number of central terms those in turn also are consumed by a large number of central documents. Following their conceptualization of recursive document centrality measures, two recursive keyword centrality measures (i.e., $v^{au}_t$ and $v^{at}_t$) were developed for each keyword $v$ in each year $t$ of the training period.
The first centrality measure considers the keyword-author bipartite relations whereas the second, considered the keyword-article relation.
In case of the first bipartite relations, the intuition behind a keyword's importance is defined by the number of central authors who, in turn, also use a large number of central keywords. 

After the initial textual keyword and data processing, we filtered out those keywords appeared in only one article.
This category denotes the specialized keywords not related to the wide majority of the scientific articles. 
With the remaining number of keywords, we constructed a keyword-author adjacency matrix $M_{AxK}$ for each year $t$ in the training period. 
It is worth mentioning that we considered the first name and last name of the authors and manually verified with the affiliation information to perform author name disambiguation. 
Although the objective of this manual author name disambiguation was to find all publications that belong to a given author and distinguish them from publications of other authors who share the same name, however, exploration of other methods for the same purpose is left for future studies.
The adjacency matrix $M$ is a binary matrix of size $|A| \times |K|$ where $A$ and $K$ denote the set of authors and keywords respectively in year $t$. 
An entry in matrix $M$ is $1$ if the author $a \in A$ uses the keyword $k \in K$ in his/her article.
Starting with an example author $a_i$ in year $t$, for each keyword $k_i$ used by this author, we can reach all other authors who also used $k_i$ in their article. 
Iterating this procedure twice,  we reach all the authors in two-hop distance from $a_i$. 
These authors used keyword(s) that is also used by author(s) sharing some keywords with author $a_i$. 
Figure ~\ref{fig:origin} demonstrates the iteration procedure with some example keywords.
This measure accumulates the number of different paths available among authors through their keyword usages.
Higher number represents that the corresponding keyword is pervasive across the research domain and thus more central and familiar to the key authors.
To calculate recursive keyword centrality in this way, two vectors $\psi_k$ and $\psi_a$ are defined recursively:
\begin{equation}
\psi_k(n,t)=\frac{\sum_{a}M(t)\psi_a(n-1,t)}{\psi_k(0,t)} , \  
\psi_a(n,t)=\frac{\sum_{k}M(t)\psi_k(n-1,t)}{\psi_a(0,t)} 
\end{equation}
with $n$ represents the number of iterations as portrayed in Figure ~\ref{fig:origin}. $\psi_k(0,t)$  and $\psi_a(0,t)$ denote the initial conditions  as $\psi_k(0,t)=\sum_{a\in A} {M}(t)$ and $\psi_a(0,t)=\sum_{k \in K} {M}(t)$. 
The values of $\psi_k$ can have different interpretations.
\begin{figure}[!h]
    % \captionsetup{justification=centering}
    \includegraphics[width=.98\textwidth, height=9cm]{{original_centrality}.pdf}
    \caption{Computation of recursive keyword centrality measure using keyword-author relations. The computation is an iterative procedure that starts at an author, $a_0$. The first iteration counts the number of authors that used a keyword which is also used by $a_0$. Then this iteration continues until it reaches the terminating condition}
    \label{fig:origin}
\end{figure}
The initial condition $\psi_k(0,t)$ denotes the degree centrality of a keyword.
For different values of $n=1, 2, 3 ...$, values of $\psi_k$ assign weights to individual keywords considering the number of authors consuming them in their articles. 
Therefore, high values of $\psi_k$ corresponds to the keywords selected by a large number of authors those used large number of such keywords.
Conversely, low values represent the keywords` specificity and relevance to limited number of research issues. 
Similar observations are also true in case of $psi_a$.
The number of iteration converged  and found stable at $n=20$.
We also attempted higher value of $n$ however. found similar recursive centrality values returned by the algorithm.
Thus, for each year $t$ in the training period, we calculated a vector of z-score normalized recursive keyword centrality values $C^{au}_t$ by following the algorithm, from the keyword-author bipartite relations.
% The centrality measures were $z$-score normalized.
Likewise, another recursive keyword centrality measure $C^{at}_t$ was constructed from the keyword-article bipartite relations in each year $t$ during the training interval. 
In addition to these recursive centrality measures, to compare the results with a traditional centrality measure, we also calculated degree centrality values of keywords $C^d_t$, extracted from the unipartite keyword-keyword relations in KCN for each year $t$.
% Degree centrality values were extracted for prediction results comparison's sake.
Future studies can calculate other centrality values to compare the results further.



==> aggregated_feature.tex <==
\subsection {Aggregated Features}
\setlabel{Aggregated Features}{sec:aggregated_feature}
In the aforementioned section, we have identified individual attributes of keywords that can  provide helpful clues about their participation in emerging relation. . 
Since, these attributes only pertain to one keyword in KCN, some aggregation functions need to be used to combine/aggregate the individual attribute values of the corresponding keywords in a pair of keywords.
To illustrate further, consider the fact that if either(or both) of the keywords are prolific or belong to the same community, it is more likely that they will co-occur.
Before aggregation, the individual measure denotes the proliferation rate of individual keyword,  its community membership, or temporal activeness (number of co-occurrences).
Aggregation of these individual features yields the aggregated features that is meaningful for the pair of keywords in dynamic link prediction.
In this study's context, we assume that the higher the aggregated feature values for a keyword pair, the more likely that those two keywords will co-occur.

% \subsubsection {Temporal community importance}
% \setlabel{Temporal community importance}{sec:heredity}	

% This is the first feature we computed for each non-connected keyword pair for the link prediction purpose.
% The objective of this feature was to capitalize both the origin information (genealogical community) and current activeness (centrality measures) of both keywords in a keyword pair.  
% In the above sections, we have defined important attributes of keywords by leveraging the properties of temporal KCNs and historical family lineage. 
% These are: firstly,  \ref{sec:rec_centrality} measures and secondly, their \ref{sec:genealogy_typology}.
% % To develop this edge-level aggregated feature, characterising keyword-pairs, we combined and aggregated these keyword features.
% % For each type of centrality measure, we multiplied keyword's corresponding centrality value with its genealogical typology (i.e., community) score.
% Chenhao Tan ~\cite{genealogy} investigated how the origin of a community connects to its future growth and demonstrated that the history of the early members allows us to understand the emergence of communities (i.e., tracing the origin of a community).
% In regards to the future community growth, the author believed that the emerging process of a community is analogous to complex contagion that requires dense connections between early adopters.
% In our case the early adopters are the members of the grandparent and parent communities.
% % Consequently, the aggregated feature for these twscores should have their community scores augmented.
% Therefore, we first multiply individual keyword's community score  with its corresponding centrality value  for each year in the training period.
% The former denotes the keyword's relation with previous year's central keyword (i.e., keyword's family lineage) and the later denotes its importance which was originally used to determine its community membership.
% This will augment the community importance scores of grandparent and parent keywords more than children and guests, and subsequently determine the individual temporal community importance score of a keyword in each training year.
% Finally, for each keyword pair, the temporal community importance score was computed by summing their aggregated individual score in each year $t$.
% Thus, the first edge-level feature at each timestamp $t$ in the training period, known as temporal community importance score for a keyword pair, can be computed as:

% \begin{align}
% \begin{split}
% &score^H_t(a,b) = g^{a}_t\cdot v^{a}_t + g^{b}_t\cdot v^{b}_t
% \end{split}
% \label{eq:typology}
% \end{align}
% where $g^{a}_t$ and $v^{a}_t$ denote the genealogical community score and the corresponding centrality score of keyword $a$.
% Thus, by considering the temporal sequences of individual community score and centrality value of both keywords,  we built a time series of this aggregated feature for each instance of non-connected keyword pair.
% Since we considered three centrality values (i.e., $v^{au}_t$,  $v^{at}_t$ and degree) for each keyword $v$ to determine its community score, the following notations will be used to denote three variants of this feature value:
% $score^H_{au}(a,b)$ to denote the temporal community importance score for an edge $(a,b)$ where recursive centrality measures of keywords $a$ and $b$ were extracted from the keyword-author relations. 
% Similarly, $score^H_{at}(a,b)$ will denote the same feature value where recursive centrality measures were extracted from the keyword-article relations.
% Finally, $score^H_{d}(a,b)$ will be used to denote the same feature value where degree centrality values of keywords $a$ and $b$ were considered.

% \subsubsection {Citation-weighted Recency}
% \setlabel{Citation-weighted Recency}{sec:cit_recency}	

% An individual keyword's citation count represent its influence factor over other keywords.
% However, domain-specific and old keywords can achieve higher citation counts then the others.
% Relative influence factor should also be brought into consideration.
% For example, old keywords accumulate more citation over time then new keywords.
% In contrast, some new keywords can gain significance quickly and acquire relatively high citation then other insignificant but old keywords.
% Therefore, we considered the temporal factors of keyword's appearances such as current or distant appearances over time. 
% Considering our training period (\eg, 2008-2014), an article published in 2008 gets more time to be cited than a article published in 2014. 
% Despite, the later one carries more impact, the former one is  weighted more based on the numbers. 
% Further, training year closer to the test period (e.g., 2014) is more significant than earlier years since recently co-appeared keywords are more likely to come together in near future, a fact known as `recency' in link prediction task ~\cite{yang2012predicting}.

% Considering the aforementioned facts on temporal significance and citation count, we constructed our second feature for keyword pairs by accommodating both temporal recency and citation counts over time.
% Since citation count and temporal recency are applicable to individual keywords, it requires to aggregate these counts for keyword-pairs.
% For each keyword pair in year $t$, we aggregated their total citation counts. 
% Further, we assigned temporal recency score depending on the appearances of both keywords in a particular year.
% The recent their appearances are, or alternatively, the closer their co-appearances towards the test year, the higher the recency score.
% Considering the keyword-pair $(a,b)$, let  $t$ denotes the training year $t \in [1, 2, 3, ... T]$, $h^u_t$ and $h^v_t$ denote the total number of citation counts of the articles in year $t$ where keywords $a$ and $b$ appears respectively, then the weighted-citation recency is calculated as follows:

% \begin{align}
% \begin{split}
% &score^W_t(a,b) =  (h^a_t + h^b_t) \cdot \gamma t 
% \end{split}
% \label{eq:recency}
% \end{align}
% Here, $\gamma$ amplifies the recency effect and its value is two if both keywords in a keyword-pair appear in a year, one if either of the keyword appear, or zero (0) otherwise. 
% $h^a_t$  will be assigned zero value if keyword $a$ does not appear in an article that received any citation.
% However, the feature value will be augmented depending on the current appearances of the keywords (i.e., multiplied by value of $t$). 
% The assumption here is that, keywords having high citation in the recent years will have high probability to appear together since they represent the recent trends.

==> genealogy.tex <==
\subsection {Genealogical Typology}
\setlabel{Genealogical Typology}{sec:genealogy_typology}

Due to prevailing preferential attachment in KCN, there exists a set of most central keywords which generally has greater influence over the structure of the network. 
It was observed that other keywords generally tend to form relations by co-appearing with these rich keywords.
To predict the future connections between keywords, this fact is needed to take into consideration.
In this study, we capitalize the idea of preferential attachment, but in a different way.
% Before describing some temporal and network characteristics of individual author selected keywords extracted from dynamic KCN, below are the description of some frequently used notations in 
\begin{table}[!h]

\begin{threeparttable}
\centering
\caption{Frequently Used Notations}
\label{notations}
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}}ll}
\toprule
Notation    & Description \\
\midrule
${k_{gp},k_p,k_c,k_g}$        & Four keyword types: {Grandparent, Parent, Children, Guest}                          \\
% $C^{au},C^{at}$	& Vectors representing recursive keyword centrality measures computed from \\ & author-keyword and article-keyword bipartite relations 	\\
$v^{au}_t,  v^{at}_t$    & Two variants of recursive centrality values for keyword $v$ at time $t$ (year) \\ & calculated from keyword-author and keyword-article bipartite relations\\
$N^{au}_{t},N^{at}_{t}$ & Sets of top $N$ central keywords in year $t$ \\ & considering the bipartite network centrality measures\\

% $t_s, t_f$ & Starting year and ending year of training time range $T$\\
\bottomrule
\end{tabular*}
\end{threeparttable}
\end{table}
\begin{figure}[!h]
    \centering
    \includegraphics[width=.9\textwidth, height=8.5cm]{{heredity_build}.pdf}
    \caption{Genealogical communities of keywords by considering a set of keywords with high recursive centrality values (i.e., $N^{au}_{t-1}$) computed from keyword-author bipartite relationships. Keywords with high centrality values at timestamp $t-1$ are designated as grandparents ($k_{gp}$ at timestamp $t$. Direct neighbours of these grandparents belong to parents ($k_p$) community, and two-hop neighbours are designated as children ($k_c$).Rest of the keywords are designated as guests ($k_g$).} 
    \label{fig:heredity_build}
\end{figure}
We defined a keyword's genealogical community score in each year that denotes it's current ancestral relation with previous year's central keywords. 
The underlying objective here was to capture the evolution of keywords over the years and lineages to their ancestry. 
Genealogy is the study of family tree and a genealogy graph is used to portray the complex evolving relation originating from the ancestors. 
Before jumping into the detail of this community definition, Table \ref{notations} provides descriptions of some notations those will be used frequently in the sections below.
In the same way, we defined a keyword's family relationship in a particular year $t$ based on it's relation with the central keywords from previous year $t-1$. 
The centrality of keywords was measured by considering two recursive centrality measures and one degree centrality.
This approach would label keywords according to the type of their ancestral relationships (e.g., grandparents, parents, child or guest) and help us understanding the impact of these relationship types in their co-occurrences.
The computation of genealogical community score is described below:

In our dynamic KCN, we defined four types of communities for keywords, namely, grandparents $(k_{gp})$, parents $(k_p)$, children $(k_c)$ and guests $(k_g)$.
Firstly, we defined the grandparents.
If we consider identifying community membership of keywords in year $t$, then grandparents $k_{gp}$ keywords are the top-$N$ central keywords from year $t-1$. 
Here, the word `central' denotes higher values of a chosen centrality measure from the three aforementioned centrality measures (i.e., two recursive and one degree centrality). 
In other words, these are the most frequent and influential keywords both in regards to the contents of metadata information (e.g.,author and article) and in forming relations with other keywords. 
We experimented with the number of grandparents ranging from $10-200$ by considering two recursive centrality measures.
Interestingly, we found that having $N\geqslant20$  grandparents in each year does not change the prediction performance (described later) significantly in both datasets.
Therefore, we designated the top $20$ keywords as grandparents by considering the centrality measures. 
In the result section, we present the recursive centrality values  $v^{au}_t$ of keywords belonging to four communities and participating in the edges during the test year (2015).
The clusters of all keywords will be evident in support of this choice.
% Replicating the same decision choice, we also keep the number of grandparents at $N=20$ by considering the degree centrality values of the keywords.
In this way, we got three sets of top-$20$ central keywords  based on our three centrality measures (i.e., $C^{au}_{t-1}$, $C^{at}_{t-1}$, and $C^{d}_{t-1}$). 
Secondly, we define the parents, children and guests.
% Let $N^{au}_{t-1}$ denotes the top-$N$ central keywords identified by using keyword-author recursive centrality measure (i.e., $C^{au}_{t-1}$). 
% These $N$ keywords from year $t-1$ are labeled as grandparents $(k_{gp})$ in the year $t$.
Keywords having direct relations (i.e., an edge is observed between them) with $k_{gp}$ are labeled as parents $(k_p)$ in the year $t$. 
Subsequently, children $(k_c)$ are the direct neighboring nodes of $k_p$ keywords but not $K_{gp}$. 
Alternatively, $k_p$ keywords are considered as common neighbours between $k_{gp}$ and $k_c$. 
Once these three communities of keywords (i.e. $k_{gp}, k_p, k_c$) are labeled, rest of the are designated as guests $(k_g)$. 
% we exclude them from the set of all keywords $(V_t)$.
% Rest of the keywords are designated as guests $(k_g)$.
These guests keywords had maximum distance from the grandparents.
In this way, we defined the genealogical communities of all keywords appearing in a particular year. 
% (as shown in Equation \eqref{eq:gp} - \eqref{eq:g}). 
In our experiment, we use top-$20$ keywords from year $(t=0)$ (i.e., 2007) for the first training year $(t=1)$ (i.e., 2008), though this year $(t=0)$ is not included within our training period. 
This fact was mentioned in the earlier section \ref{sec:data_acquisition}.
\begin{figure}[!h]
\begin{subfigure}{.33\textwidth}
    \includegraphics[width=1\textwidth]{{2011sar}.pdf}
    \caption{$G_s$: 2011 (keyword-article)}
    \label{fig:2011oar}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
    \includegraphics[width=1\textwidth]{{2011sau}.pdf}
    \caption{$G_s$: 2011 (keyword-author)}
    \label{fig:2011oau}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
    \includegraphics[width=1\textwidth]{{2011sde}.pdf}
    \caption{$G_s$: 2011 (degree)}
    \label{fig:2011ode}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
    \includegraphics[width=1\textwidth]{{2014sar}.pdf}
    \caption{$G_s$: 2014 (keyword-article)}
    \label{fig:2014sar}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
    \includegraphics[width=1\textwidth]{{2014sau}.pdf}
    \caption{$G_s$: 2014 (keyword-author)}
    \label{fig:2014sau}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
    \includegraphics[width=1\textwidth]{{2014sde}.pdf}
    \caption{$G_s$: 2014 (degree)}
    \label{fig:2014sde}
\end{subfigure}
\caption {\protect\raggedright Temporal variations of genealogical traits demonstrated by keywords depending on the centrality measures used in $G_o$ dataset. 
All network snapshots are timestamped including the centrality measure used to identify the genealogical traits.
The color codes represent the genealogical communities of keywords: red (grandparent), green (parent) and blue (child). 
The size of the node represents to the keyword's corresponding centrality measures. }
\label{fig:h_variation}
\end{figure}
Next, we assign each keyword a score according to its genealogical community membership. 
The successive order of keyword's genealogical community score is: $score(k_{gp}) >> score(k_p)> score(k_c)> score(k_g)$.
Here, $k_{gp}$ keywords are considered as the most influential keywords in the KCN of a particular year. 
% Although, this does not necessarily mean that grandparents will have most of the connections since top central keywords in the previous year will not necessarily be on the top in the current year. 
% Despite the trivial quantity of these influential keywords every year, individually these were found to form most relations with others.

Being most influential in the previous year, they are assigned the highest score in the current year. 
Scores for the other three keyword types: $k_p$,$k_c$,$k_g$ were defined according to their distance from the grandparents $k_{gp}$. 
Being the most distant ones, $k_g$ (guests) are assigned with lowest community score. 
% The process of labeling all keywords for a particular year $t$ using previous year's central keywords and assigning the keyword's genealogical community scores is depicted in figure \ref{fig:heredity_build}. 
The process of assigning a keyword's genealogical community scores is depicted in figure \ref{fig:heredity_build}.
The relative size of each keyword in this figure represents the weight of the score (i.e. greater size for higher value). 
% Likewise, we computed two more sets of genealogical scores for each keyword using $N^{at}_{t-1}$ and $N^{d}_{t-1}$.
In this figure, $N^{au}_{t-1}$ denotes the set of ton-$N$ central keywords by considering recursive centrality values $v^{au}_t$ extracted from keyword-author relations.

Considering three sets of centrality measures of keywords (i.e., $v^{au}_t,  v^{at}_t$  and $v^{d}_t$), a keyword belonging to one genealogical community (\eg, grandparent) in one set, might belong to different community(\eg, parent) in another.
This effectively means that if a keyword becomes grandparent by considering the $v^{au}_t$, it may not necessarily be true by considering the other centrality measures (i.e., $v^{at}_t$ or degree centrality).
Likewise, considering the same centrality measure, a keyword can belong to different genealogical community in different year.
In Figure \ref{fig:h_variation}, a comparative representation of these variations are presented  for some keywords in $G_s$ datasets.
In this figure, top two rows present network snapshots in $G_s$ considering six keywords (i.e., \textit{\textbf{atherosclerosis, morbid obesity, diagnosis, excessive daytime sleepiness, behavior, and compliance}}).
(It is evident that there exists some commonality of keywords in both datasets since some of these keywords resemble to those in the $G_o$ dataset.
Since the commonality is out of the scope of this study, we leave it for future studies where domain experts can contribute towards literature based discovery related to these two domains together.)
The first row in this figure presents the network snapshots in the year 2011 and the second presents snapshots in the year 2014.
In each row, the left snapshot presents the genealogical typologies (i.e., communities) of keywords identified by considering the recursive centrality (i.e., $v^{at}_t$) from keyword-article bipartite relations.
The snapshots in the middle column present the genealogical typologies of keywords identified by considering the recursive centrality  (.i.e., $v^{au}_t$) from keyword-author bipartite relations.
The right column presents the similar by considering the keyword's degree centrality.
Color codes represent different types of the keywords: grandparent (red), parent (green), and child (blue).  
The sizes of the nodes and labels denote corresponding centrality values.
It is observable that keywords can belong to different communities in different years by considering different centrality measures used in this study.
Consider the genealogical communities of the keyword \textit{diagnosis}.
In the year 2011, it was designated as `grandparent' by considering  $v^{at}_t$, whereas considering the same centrality measure, it belonged to `parent' community in 2014.
Surprisingly, the later is also true (`parent') when recursive centrality measure $v^{au}_t$ was considered in the year 2011.
Similar observations are evident in case of the keyword \textit{behaviour}
There are some domain-specific keywords (\eg   \textit{sleep}, \textit{apnea},\textit{ obesity}) which were found as `grandparents' in all centrality variants since they are the representative keywords of the respective domain. .


\begin{table}[!h]
    % \tabcolsep 5pt
    % \small
\begin{threeparttable}
\centering
\caption{Number of nodes (keywords) according to different genealogical typologies (i.e., communities) defined in this study and edges (keyword pairs) between different typologies of keywords. $GP$ represents the grandparents keywords, $P$ represents the parents, $C$ represents the children and $G$ represents the guests keywords. Similarly, $E_{P}$ denotes the edges between parent keywords, and $E{GP \leftrightarrow P}$ denotes the edges between grandparent and parent keywords.}
\label{table:gr_type}
\begin{tabular}{lrrrrrrrrrrrrrrr}
\toprule

Year &   $P$ &  $C$  &  $G$ &    $E_{GP\leftrightarrow P}$ &  $E_{GP \leftrightarrow C}$ & $ E_{GP \leftrightarrow G}$ & $E_P$ &  $E_{P \leftrightarrow C}$ & $E_{P \leftrightarrow G}$ & $E_C$ &  $E_{C \leftrightarrow G}$ & $E_G$\\
\midrule
& & & & & &$G_s$\\
 \midrule
2008 &      197 &   95 &  147 &         66 &      27 &      52 &   91 &     70 &     86 &   15 &     46 &   26 \\
2009 &     179 &   84 &  187 &           65 &      32 &      56 &   89 &     62 &     95 &   13 &     30 &   32 \\
2010 &     189 &   98 &  189 &            70 &      29 &      58 &   97 &     48 &    101 &    9 &     34 &   26 \\
2011 &     225 &  116 &  175 &           81 &      29 &      52 &  112 &     64 &    115 &   13 &     41 &   25 \\
2012 &    243 &  127 &  194 &          103 &      51 &      49 &  151 &     94 &    104 &   19 &     49 &   23 \\
2013 &    273 &  167 &  174 &          99 &      45 &      52 &  156 &    121 &    114 &   23 &     49 &   24 \\
2014 &    235 &  156 &  172 &       100 &      53 &      35 &  141 &    140 &     66 &   31 &     64 &   27 \\
\midrule
& & & & & &$G_o$\\
\midrule
2008 &    1765 &  430 &  141 &          679 &     185 &      67 &  3729 &   1083 &    283 &   72 &     38 &    3 \\
2009 &     1614 &  360 &   98 &          664 &     157 &      32 &  3626 &    968 &    242 &   63 &     44 &    0 \\
2010 &     1752 &  409 &  117 &           556 &     153 &      43 &  4072 &   1148 &    302 &   69 &     25 &    5 \\
2011 &     1963 &  334 &   91 &          665 &     125 &      27 &  4628 &    925 &    258 &   37 &     34 &   10 \\
2012 &     2109 &  368 &   82 &           757 &     131 &      26 &  5723 &   1024 &    190 &   48 &     12 &    1 \\
2013 &     2117 &  370 &   75 &         726 &     148 &      41 &  5582 &   1375 &    211 &   73 &     30 &    1 \\
2014 &    2252 &  793 &  155 &       869 &     323 &      51 &  6903 &   2200 &    310 &  193 &     54 &    4 \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table}

\subsection {Genealogical Community and KCN Evolution}
\setlabel{Keyword's Community and KCN Evolution}{subsec:type_evolution}

In Table \ref{table:gr_type}, basic statistics of nodes (keywords) and different types of edges (keyword co-occurrences) formed between keywords belonging to different genealogical communities are presented. 
% the list of keywords according to different genealogical typologies (communities) and edges among these keywords are presented for each year of the training period.
% As described in section ~\ref{sec:genealogy_typology}, we classified author selected keywords into four different communities based on their family lineage: grandparents, parents, children and guests.
% It is noteworthy that considering the recursive keyword centrality measures, we always selected top-20 keywords from the time $t-1$ acting as the grandparents at time $t$.
In this table, we ignored the grandparent keywords since for each year it was the top-20 keywords from the previous year.
Consequently, edges among the grandparents keywords in subsequent years were also ignored since they were trivial in comparison to the other types of edges.
In both datasets, we found that edges among keywords belonging to the parent community dominate in numbers.
This fact is correlated with the increase of number of edges between grandparents and parents over time.
% This fact further signifies the preferential attachment phenomena
% Similarly, despite the number of grandparents was trivial, we observed that the number of edges between grandparents and parents also increased over time.
The children and guest keywords tend to form edges with parents more than the grandparents.
This chronology of descendants not only helped us understand the temporal trends of topics and research hypotheses developments but also attribute specificity in preferential attachment.
For example, in absence of such typologies, we would consider grandparents and parents keywords not only in the same category and but also the richest since these would acquire most of the emerging edges.
From this table, we can also observe contrasting phenomenon which signifies the fact that the richest does not always remain so as they grow oldest.
Considering the sizes (i.e., number of articles and keywords) of both datasets, $G_s$ harbours more guest keywords and edges.
However, the ratio of edges between children and guest keywords are similar in both datasets.
Such classification on genealogical traits will allow us to comprehend the evolutionary growth of KCNs better and thus help in science mapping.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\textwidth]{{test_relation}.pdf}
    \caption{Percentage of different types edges among keywords from different genealogical communities with respect to the total number of edges in the test year (i.e., 2015)}
    \label{fig:test_relation}
\end{figure}

In Figure ~\ref{fig:test_relation}, we observe how this ancestral relationships helped us to classify the edge types in the test year (i.e., 2015).
In this figure, we present the percentage of different types of edges, as presented in Table \ref{table:gr_type}, with respect to the total number of edges.
It is evident from this figure that the keywords belonging to the parent community play crucial roles in emerging relations than any other keyword types.
In both datasets, the parent keywords dominate in attracting both descendants and antecedents to form emerging relations.
